Trajectory prediction for heterogeneous agents: A performance analysis on small and imbalanced datasets

Robots and other intelligent systems navigating in complex dynamic environments should predict future actions and intentions of surrounding agents to reach their goals efficiently and avoid collisions. The dynamics of those agents strongly depends on their tasks, roles, or observable labels. Class-conditioned motion prediction is thus an appealing way to reduce forecast uncertainty and get more accurate predictions for heterogeneous agents. However, this is hardly explored in the prior art, especially for mobile robots and in limited data applications. In this paper, we analyse different class-conditioned trajectory prediction methods on two datasets. We propose a set of conditional pattern-based and efficient deep learning-based baselines, and evaluate their performance on robotics and outdoors datasets (TH\"OR-MAGNI and Stanford Drone Dataset). Our experiments show that all methods improve accuracy in most of the settings when considering class labels. More importantly, we observe that there are significant differences when learning from imbalanced datasets, or in new environments where sufficient data is not available. In particular, we find that deep learning methods perform better on balanced datasets, but in applications with limited data, e.g., cold start of a robot in a new environment, or imbalanced classes, pattern-based methods may be preferable.

==> contents/0_abstract.tex <==
\begin{abstract}
%In domains such as autonomous driving and robotics, intelligent mobile systems need to foresee the movements of heterogeneous agents to ensure seamless interactions and safe operation. Heterogeneous agents are categorized into classes because they share the same space with different motion patterns. Class-based trajectory predictors aim to incorporate the class information to ensure more accurate predictions. In this work we first adapt deep learning and Maps of Dynamics methods with the class information of the agents. Then, we comprehensively analyse each method on two datasets: Stanford Drone Dataset for road users and TH\"{O}R-MAGNI dataset tailored for robotic services and industrial environments. Our experiments show that globally, class information promotes more effective trajectory predictors regardless of their nature (learning or non-learning). We also show that non-learning based methods are preferred over deep learning based methods for certain applications. This preference is contingent on factors related to the specific application, such as the amount of data available during training or the amount of samples per class, providing crucial insights into optimal method selection for the heterogeneous trajectory prediction task.
%
Robots and other intelligent systems navigating in complex dynamic environments should predict future actions and intentions of surrounding agents to reach their goals efficiently and avoid collisions. The dynamics of those agents strongly depends on their tasks, roles, or observable labels. Class-conditioned motion prediction is thus an appealing way to reduce forecast uncertainty and get more accurate predictions for heterogeneous agents. However, this is hardly explored in the prior art, especially for mobile robots. In this paper, we analyse different class-conditioned trajectory prediction methods on two datasets. We modify several popular types of pattern-based and deep learning methods to include prior class labels, and evaluate their performance on robotics and outdoors datasets (TH\"{O}R-MAGNI and Stanford Drone Dataset). Our experiments show that all methods improve accuracy in most of the settings when considering class labels. We further observe that there are important differences when learning from imbalanced datasets, or in new environments where sufficient data is not available. In particular, we find that deep learning methods perform better on balanced datasets, but in applications with limited data,
e.g., cold start of a robot in a new environment, or imbalanced classes, pattern-based methods are preferable.
\end{abstract}

==> contents/1_intro.tex <==
\section{INTRODUCTION} \label{section-intro}

% 1) the hook
% 2) the gap
% 3) our study
% 4) contribution and conclusion
% 5) outline 

%radar/spider plot vertex -> data % two plots for high balance and low balanced the range is the accuracy

% lower data regimes (for instance during cold-start of a robot in a previously unseen environment) -> use (c)MoD
% higher the amount of data -> DL models do the job
% if you want multiple outputs and natural datasets where the classes are imbalanced -> (c)MoDs


% Paragraph 1: 
% Motion prediciton is important for robotics -> safety, etc.
% Deep Learning has been used 
% Classes are important for both AD and robotics applications; it improves the prediction of trajectories [ICCV]


% Paragraph 2: 
% Robotics applications have further specifities that may affect the choice of prediction methods such as:
% - during cold-start of a robot in a previously unseen environment, there is no much data and the question is are the 
% current methods accounting for this particularity? In specific, are deep learning-based methods performing in these 
% settings? Other methods, like CVM does not work very well for complex datasets as seen in [ICCV]; can we introduce 
% a novel non-learning based approach that accounts for classes and performs comparatively to deep-learning based methods?


% Paragraph 3 - our study
% - can we introduce an analysis that tells the reader which method to use in which occasion? 
% - for that we analyse deep learning based methods and a non learning approach based on MoDs; we introduce the class-based variant 
% in this paper


% Paragraph 4- Contribution and conclusion
%  - extension on previous work on deep learning-based methods for class-based trajectory prediction:
    % - transformers everywhere
    % - non-learning based approach for class-based trajectory prediction based on maps of dynamics
% - an anlysis of multivariate methods for heterogeneous trajectory prediction in different datasets
% - empirically grounded indications of which method to use in which case

%TODO: conclusion paragraph

Reliable and safe robot navigation in dynamic human-centered environments relies on anticipating the future 
behavior of other agents. In several domains, including autonomous driving and industrial mobile 
robotics, the motion planner must proactively consider the future positions 
of many heterogeneous agents to maintain safety standards~\cite{teja21}. In 
autonomous urban driving, 
various entities with distinct dynamic patterns such as pedestrians, bicyclists, and cars navigate in a shared space.
In industrial environments, humans engaged in different tasks, such as transporting objects, interacting 
with robots, or walking in groups, may also present different motion patterns within the same spatial 
layout~\cite{almeida23}. The diversity of agents and their corresponding motion patterns poses significant 
challenges for current trajectory predictors~\cite{fang22}, leading to high forecast uncertainty, lower prediction accuracy, and thus to overly conservative motion planning~\cite{heuer2023proactive}. 

\begin{figure}[!t]
   \centering
   \includegraphics*[width=\linewidth]{figures/ral_cover_last2.pdf}
   %\caption{Average Displacement Error on various data settings. \textbf{Top:} Performance of a class-conditioned pattern-based method (cMoD in green) and deep learning methods (cLSTM, cTF, cGAN and cVAE). Deep learning methods are generally more effective for balanced (Magni-S3A) and high-data regimes settings. \textbf{Bottom:} Two examples of the extremes of training data regimes: 10\% training ratio on MAGNI-S3A and 90\% training ratio on SDD show that class-conditioned methods outperform unconditioned counterparts (LSTM, TF, GAN, VAE, and MoD).}%Radar plot illustrating the percentage of training data on the vertices and error performance across radial grid lines. The non-learning-based method (cMoD) outperforms deep learning methods in low-data regimes and in imbalanced datasets (SDD).} 
   \vspace*{-8mm}
   \caption{Average Displacement Error of class-conditioned trajectory prediction methods across balanced and imbalanced datasets. 
   \textbf{Top:} In balanced datasets, at 
   low data regimes (10\% train set ratio), the pattern-based method (cMoD) is more accurate than deep learning methods (\textbf{left}). In imbalanced datasets, 
   cMoD is more accurate than deep generative models (\textbf{right}). Thus, the pattern-based method, cMoD, is more suitable 
   for low training data regimes and imbalanced datasets than deep learning methods. \textbf{Bottom}: Class-conditioned 
   methods (c***) consistently outperform their unconditional counterparts across both datasets.}
   \label{fig:cover}
\vspace*{-6mm}
\end{figure}

In the context of mobile robots in dynamic environments, prior art has hardly explored class-aware prediction approaches, 
which is particularly evident given that human motion datasets with class or activity labels are still rare~\cite{schreiter2022magni}. Moreover, 
existing heterogeneous trajectory prediction methods tailored for autonomous driving do not transfer well to robotics settings, as they depend on domain-specific contextual features~\cite{chandra19}. 
Furthermore, robotics applications present unique challenges, such as the cold-start scenario, 
where a robot enters a previously unseen environment with limited data~\cite{cui21} and continuously navigates it. Additionally, various applications may feature non-uniform class distributions, leading to decreased performance of deep learning-based trajectory prediction methods~\cite{almeida22}.
Our central research question is whether class-conditioned prediction methods can address applications characterized by a low data regime and/or class-imbalanced datasets, and if so, under which specific circumstances. %This question underscores the need for a comprehensive analysis of trajectory prediction methods that explicitly consider the class of agents.% involved in different datasets.


%For instance, traditional methods such as the Constant 
%Velocity Model may work well on less complex datasets~\cite{scholler20}, but perform poorly in complex scenarios such as industrial environments as shown in~\cite{almeida23}. 
%This disparity underscores the need for a comprehensive analysis and comparison of trajectory prediction methods that explicitly 
%consider the class of agents involved in different datasets.


% In order to facilitate development and application of motion prediction methods for autonomous systems in realistic unstructured environments ...
In this paper, we present an in-depth study of class-conditioned trajectory prediction methods
%, aiming to provide insights into their performance
under different conditions. We extend a pattern-based approach CLiFF-LHMP~\cite{zhu2023clifflhmp}, which uses Maps of Dynamics~\cite{tomasz_survey23} (MoD), to introduce a class-conditioned variant, and similarly adapt several deep learning methods to include class labels.
We assess their performance across diverse training data conditions, considering both balanced and imbalanced datasets 
(where class proportions are uniform and non-uniform, respectively), and various amounts of training data. The study of 
imbalanced datasets is significant as deep learning methods may struggle to predict underrepresented classes, 
which is particularly impactful when these classes represent vulnerable road users such as pedestrians. The study of various training data 
amounts reflects a practical challenge in mobile robotics, where the system is deployed in new environments 
with limited acquired data yet requiring anticipation of other agents' movements for safe navigation.
We analyze heterogeneous agents prediction in two distinct datasets: the Stanford Drone Dataset (SDD)~\cite{robicquet16}, 
which focuses on road users outdoors, and the TH\"{O}R-MAGNI dataset~\cite{schreiter2022magni}, which captures an mockup indoor industrial 
environment with mobile robots and human agents. 
Through this comparative study, we aim to show the preferred methods for specific settings, highlighting their performance in 
different data 
regimes and class-imbalanced datasets.
\cref{fig:cover} outlines the main results of our study. 
 %we present in the remainder of this paper.

\begin{comment}
\begin{itemize}
    \item We introduce a novel class-conditioned MoD approach and adapt four common deep learning approaches for motion prediction (LSTM, VAE, TF and GAN) to consider class or activity labels.
    \item We analyze performance of these methods across the indoor mobile robot and outdoor mixed traffic datasets.
    \item We show that ... (some specific important conclusions)
\end{itemize}
\end{comment}

In summary, we make the following contributions:

\begin{itemize}
    \item We extend previous deep generative models with transformer-based encoders for trajectory prediction and introduce a semantic extension of an MoD approach.
    %\item We analyse the performance of a pattern-based method (CLiFF-LHMP) and four deep learning approaches that consider class or activity labels in indoor mobile robot dataset and outdoor mixed traffic scenarios.
    \item We analyse the performance of deep learning methods and an MoD approach that consider activity labels or agent classes in an indoor mobile robot dataset and outdoor mixed traffic scenarios.
    \item %We show that class-conditioned methods outperform their unconditional counterparts. In addition, we show that MoD approaches are preferable over the deep learning methods for low data regimes and class imbalanced datasets.
    We show that class-conditioned methods outperform their unconditional counterparts. In addition, we show that MoD approaches are preferable over the deep learning methods for low data regimes and class imbalanced datasets.
\end{itemize}

==> contents/2_related_work.tex <==
\section{RELATED WORK} \label{section-relatedwork}

\subsection{Motion Prediction for Heterogeneous Agents}


The task of heterogeneous trajectory prediction involves estimating the future positions of an agent based on an observed trajectory, augmented by features describing the agent class, and optionally incorporating additional contextual factors, such as environmental obstacle maps. Deep learning techniques have been widely applied to solve this problem~\cite{chandra19,unin_21_zheng,adaptive_23_geng}, in particular, by using Graph Neural Networks 
in the context of Autonomous 
Driving~\cite{ma2019trafficpredict,salzmann20,Rainbow2021SemanticsSTGCNNAS,unin_21_zheng,heat_22_mo}. However, methods developed for predicting the trajectories of road agents do not transfer their assumptions when applied to other 
environments, such as workplace environments. For instance, \emph{TraPhic}~\cite{chandra19} uses the shape of the road agent 
as a discriminative input feature for the various classes, a strategy that does not scale well to datasets with diverse human activities, such as TH\"{O}R~\cite{rudenko2020thor} or TH\"{O}R-MAGNI~\cite{schreiter2022magni}. Conversely, \emph{HAICU}~\cite{ivanovic22} uses the output of the perception 
module as a representation of the road agent's class, incorporating a continuous label distribution instead of a discrete value as the agent's type.

Alternative approaches involve individual deep learning modules for each agent 
class~\cite{ma2019trafficpredict,heat_22_mo,adaptive_23_geng} to account for the heterogeneity of the dataset. 
These methods require individual encoders and/or decoders for each class, which presents scalability challenges as the number of classes increases. 
\emph{Semantics-STGCNN}~\cite{Rainbow2021SemanticsSTGCNNAS} addresses imbalanced class proportions in 
heterogeneous motion trajectory datasets through a class-balancing loss function, yet this strategy 
struggles to achieve top performance in all classes.
To address issues of deep learning methods due to imbalanced datasets, we propose a class-conditioned MoD-based method that is significantly less sensitive to class proportions than deep learning approaches and thus improves on its unconditional counterpart.% in datasets with non-uniform class proportions.
% sacrifices performance on the most representative class.

In this paper, we conduct an analysis of class-conditioned methods that are agnostic to the scene environment, allowing for applicability across different settings. 
Specifically, we evaluate four deep learning models and a Maps of Dynamics method~\cite{zhu2023clifflhmp}, along with their respective conditional 
counterparts, on two datasets containing human motion trajectories (TH\"{O}R-MAGNI) and road agent trajectories (SDD). We argue these methods are well-suited for application in new environments to support safe mobile robot navigation.

\subsection{Heterogeneous Motion Trajectory Datasets}

% ViRAT 2011
% UCLA 2015
% sdd 2016
% L-CAS 2017
% Argoverse 2019
% Mogaze 2020
% THOR 2020
% JRDB-Act 2022
% Magni 2023
Motion trajectory datasets reflect a variety of factors that describe the dynamics of the agents' movements. These factors commonly relate to (1) agent-agent interactions~\cite{salatiello21, kothari23}, 
providing insights into the study of dynamic social interactions; 
(2) agent-environment interactions~\cite{kratzer_mogaze_2021}, describing specific environment-related events in trajectory data
or activities performed by the agent; (3) human-robot interaction (HRI)~\cite{karnan2022socially} 
supporting the research of effective methods for social navigation of robots in human-centered environments. This paper focuses on the analysis of trajectory prediction methods on
heterogeneous motion trajectory datasets containing various classes of agents. These classes include entities such as cars, pedestrians, and bicyclists in a road environment~\cite{robicquet16}, 
or human activities that influence the dynamics of human motion in a working environment~\cite{schreiter2022magni}.

Heterogeneous human motion datasets have been gathered across diverse environments, including road 
scenes~\cite{argoverse19,argoverse21}, university campuses~\cite{robicquet16,lcas_17,ehsan22}, surveilled 
outdoor areas~\cite{virat_11,ucla_15}, and indoor settings~\cite{rudenko2020thor,schreiter2022magni,kratzer_mogaze_2021}. 
In this paper, we tested our prediction methods on two datasets:
the well-established outdoor SDD~\cite{robicquet16} and the novel indoor TH\"{O}R-MAGNI dataset~\cite{schreiter2022magni}. We chose SDD and TH\"{O}R-MAGNI due to their distinct settings: imbalanced outdoor road agents and balanced human tasks in a robotics environment, respectively.









==> contents/3_methods.tex <==
\section{METHODS} \label{section-methods}
%In this section, we introduce the problem statement and present class-conditioned motion prediction methods based on deep learning models and maps of dynamics. 
\subsection{Problem Statement}
We frame the task of predicting the future trajectory of an agent as inferring a sequence of future states. With the input of an 
observation sequence $X$, and the class of the agent $c$, the task is to predict the sequence of future 
states $\mathcal{T}$. A state $s$ of an agent is represented by the 2D Cartesian coordinates $(x,y)$ and the corresponding velocity vector $(v_x,v_y)$, i.e., $s = (x,y,v_x,v_y)$. Velocity is composed of speed and orientation. After observing $O_p$ time steps, future states are predicted over $T_p$ prediction time steps, 
where $O_p = |X|$ and  $T_p = |\mathcal{T}|$.


\subsection{Deep Learning Models}

In this section, we present the deep learning methods to compare on the task of predicting motion trajectories considering agent classes. This comparison includes both single-output trajectory predictors (one prediction per observed trajectory), namely Long Short-Term Memory (LSTM), specifically the RED method~\cite{becker18}, and Transformer-based, denoted by TF~\cite{almeida23}, as well as 
 multiple-output approaches (multiple predictions per observed trajectory), including Generative Adversarial Networks (GANs) and Variational Autoencoders (VAEs). We use the single-output methods, RED and TF, and their respective class-conditioned counterparts cRED and cTF, as outlined in~\cite{almeida23}. Multiple-output approaches, GAN, VAE, and their respective conditioned counterparts cGAN and cVAE, replace the LSTM-based temporal feature extractors used in~\cite{almeida23} with Transformers-based encoders~\cite{vaswani17} (datails below). All unconditional deep 
 learning methods take as input the state $X$, usually given by the 2D Cartesian positions concatenated with the 2D velocity vector, and output 
 $\hat{Y}$, a sequence of future velocity vectors in the 2D space. Conditioned counterparts also include the class 
 of the agent provided by the dataset as an additional input.

% TODO fix the size
\begin{comment}
 \begin{figure}[!t]
  \centering
  \begin{tikzpicture}[
    >=Stealth,
    node distance=1.5cm,
    normalbox/.style={draw=black, rectangle, minimum width=1.5cm, minimum height=0.8cm, align=center},
    bigbox/.style = {draw=black, thick, fill=green!25, rounded corners, rectangle, minimum width = 4cm, minimum height = 4cm},
    box3/.style = {minimum size=0.2cm, rounded corners, draw=green!25, fill=blue!10},
    box2/.style = {minimum size=0.2cm, rounded corners, draw=green!25, fill=yellow!10},
    arrow/.style={->, thick, >=stealth},
]

  % Input embeddings
  \node[inner sep=0, anchor=center] (input) at (-5,0) {$X$};
  \node[normalbox, right=0.75cm of input] (mlp_emb) {MLP};
  % \node[inner sep=0, anchor=center,  above=0.1mm of mlp_emb] (emb_tex) {Input Emb.};

  % Positional encoding
  \node[normalbox, right=0.75cm of mlp_emb] (pos1) {Positional\\Encoding};

  % Layer
  % \node[inner sep=0, anchor=center,  below=0.75cm of pos1] (trans_tex) {Transformer Encoder};
  % \node[bigbox, below=1mm of trans_tex](trans_enc) {};
  \draw[fill=green!10] (-4.5,-0.75) -- (-4.5,-4.5) -- (-1.9,-4.5) -- (-1.9,-0.75) -- cycle;
  

  \node[box3](plus)  at (-2.5,-2.1) {Add.};

  \node[box3, below=1.5cm of plus](plus2) {Add.};
  \node[box2, left=0.40cm of plus](mha) {MHA};
  \node[box2, above=0.40cm of mha](ln) {LN};
  \node[box2, left=0.40cm of plus2](ffn) {FFN};
  \node[box2, above=0.40cm of ffn](ln2) {LN};
  \node[below=1cm of plus2] (tf) {Temporal Features};

  \draw[arrow] (input.east) to[out=0, in=180] (mlp_emb.west);
  \draw[arrow] (mlp_emb.east) to[out=0, in=180] (pos1.west);
  % \draw[arrow] (pos1.south) to[out=270, in=90] (trans_tex.north);
  \draw[arrow] (plus2.south) to[out=270, in=90] (tf.north);

  % \draw[arrow] (pos1.south) to[out=-135, in=45] (plus.north);
  \draw[arrow] (pos1.south) -- ++(0,-0.15) -| (plus.north); 
  \draw[arrow] (pos1.south) -- ++(0,-0.15) -| (ln.north);


  \draw[arrow] (plus.south) to[out=270, in=90] (plus2.north);
  \draw[arrow] (ln.south) to[out=270, in=90] (mha.north);
  \draw[arrow] (mha.east) to[out=0, in=180] (plus.west);
  \draw[arrow] (plus.south) to[out=-135, in=45] (ln2.east);
  \draw[arrow] (ln2.south) to[out=270, in=90] (ffn.north);
  \draw[arrow] (ffn.east) to[out=0, in=180] (plus2.west);
  
  \end{tikzpicture}
    \caption{Transformer encoder system.}
    \label{fig:tf_mec}
    \vspace*{-6mm}
\end{figure}
\end{comment}


\subsubsection{Single-Output Trajectory Predictors} The first step is embedding the input sequence $X$ using a 
 Multi-Layer Perceptron (MLP) network (see \cref{fig:sing_out_overview}). Additionally, cRED and cTF embed the integer class label $c$ with an embedding layer. Subsequently, for RED and cRED, the embedded input vector 
 passes through an LSTM layer, while for TF and cTF, the encoded input vector undergoes a Transformer-based encoder (see \cref{fig:tf_mec}). Lastly, an MLP-based decoder generates the predicted sequence of velocity vectors from the vector 
 encoded by the temporal feature extractors (i.e., LSTM and Transformer-based encoder). In the conditional variants (cLSTM and cTF), we concatenate the temporal features with the embeddings of each trajectory's class and pass the resulting vector to the decoder. 
 We train single-output networks with the Mean Squared Error (MSE) loss:
\begin{equation}
      L_{T}(P, \hat{P}) = \frac{1}{T_{p}} \sum_j^{T_p} \lVert p^j -\hat{p}^j  \rVert_2,
\label{eq:l_traj}
\end{equation}
%
where ${P}$ represents the ground truth future trajectory, $\hat{P}$ the estimated sequence of positions, $p^{j}$ the ground truth position at time step $j$ and $\hat{p}^j$ the corresponding predicted position.
%

\begin{comment}
\begin{figure}[!t]
  \centering
  \tikzset{myLine1/.style = {->, thick, >=stealth},
    mynarrownodes/.style = {node distance=0.75cm and 0.3cm},
    }
  \tikzstyle{bigbox} = [draw=blue!50, thick, fill=blue!20, rounded corners, rectangle]
  \tikzstyle{box} = [minimum size=0.2cm, rounded corners,rectangle split,rectangle split parts=2, inner sep=0.1ex, fill=gray!10]
  \tikzstyle{box3} = [minimum size=0.2cm, rounded corners,rectangle split,rectangle split parts=3, inner sep=0.1ex, fill=gray!10]
  \begin{subfigure}{0.48\columnwidth}
    \centering
      \begin{tikzpicture}
      \node[inner sep=0, anchor=center] (input) at (-4,2) {$X$};
      
      \matrix[below=0.3cm of input, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox, every node/.style=box3](lstm) {
            \node(embedding){\footnotesize{\textbf{Embedding}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
            \\  \node(encoder){\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{LSTM} \nodepart{third} \scriptsize{Transformer}}; 
            \\ \node(decoder){\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; \\
        };

        \node[inner sep=0, anchor=center, below=0.3cm of lstm] (output) {$\hat{Y}$};
        
        \draw[myLine1] (embedding.south) to[out=-90, in=90] (encoder.north);
        \draw[myLine1] (encoder.south) to[out=-90, in=90] (decoder.north);
        
        \draw[myLine1] (input.south) to[out=-90, in=90] (lstm.north);
        \draw[myLine1] (lstm.south) to[out=-90, in=90] (output.north);
      
      \end{tikzpicture}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.48\columnwidth}
    \centering
      \begin{tikzpicture}
      \node[inner sep=0, anchor=center] (input) at (-4,2) {$X$};
        \matrix[below=0.3cm of input, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox, every node/.style=box3](lstm) {
          \node(embedding){\footnotesize{\textbf{Embedding}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
          \\  \node(encoder){\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{LSTM} \nodepart{third} \scriptsize{Transformer}}; 
          \\ \node(decoder){\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; \\
        };
        \node[inner sep=0, anchor=center, right=0.20cm of lstm] (concat) {$\oplus$};
        \node[inner sep=0, anchor=center, right=0.95cm of lstm] (role) {$c$};
        \node[inner sep=0, anchor=center, below=0.3cm of lstm] (output) {$\hat{Y}$};

        \draw[myLine1] (embedding.south) to[out=-90, in=90] (encoder.north);
        \draw[myLine1] (encoder.east) to[out=0, in=180] (concat.west);
        \draw[myLine1] (role.west) to[out=180, in=0] (concat.east);
        \draw[myLine1] (concat.south) to[out=-90, in=0] (decoder.east);
        
        
        \draw[myLine1] (input.south) to[out=-90, in=90] (lstm.north);
        \draw[myLine1] (lstm.south) to[out=-90, in=90] (output.north);
      
      \end{tikzpicture}
  \end{subfigure}
\caption{Single-output unconditional (left) and conditional methods (right).}%The input state, $X$, is embedded with a MLP. Then, we 
%extract temporal features with LSTM (for RED and cRED models) or with a Transformer-based encoder (for TF and cTF models). Finally, the decoder takes as input 
%the temporal features and produces the future velocity vector, $\hat{Y}$. The conditional methods (right) concatenate the embedded agent class to 
%the temporal features and proceed to the decoding stage.}
\label{fig:sing_out_overview}
\vspace*{-6mm}
\end{figure}
\end{comment}

\begin{figure}[!t]
 \tikzset{myLine1/.style = {->, thick, >=stealth},
    mynarrownodes/.style = {node distance=0.75cm and 0.3cm},
    }
  \tikzstyle{bigbox} = [draw=blue!50, thick, fill=blue!20, rounded corners, rectangle]
  \tikzstyle{box} = [minimum size=0.1cm, rounded corners,rectangle split,rectangle split parts=2, inner sep=0.1ex, fill=gray!10]
  \tikzstyle{box3} = [minimum size=0.1cm, rounded corners,rectangle split,rectangle split parts=3, inner sep=0.1ex, fill=gray!10]
    \centering
      \begin{tikzpicture}
      \node[inner sep=0, anchor=center] (input) at (-4,0) {$X$};
      \matrix[right=0.75cm of input, row sep=0mm, column sep=2.5mm, inner sep=1mm, bigbox, every node/.style=box3](lstm) {
            \node(embedding){\footnotesize{\textbf{Embedding}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
            &  \node(encoder){\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{LSTM} \nodepart{third} \scriptsize{Transformer}}; 
            & \node(decoder){\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; \\
        };

        \node[inner sep=0, anchor=center, right=0.75cm of lstm] (output) {$\hat{Y}$};

        \draw[myLine1] (embedding.east) to[out=0, in=180] (encoder.west);
        \draw[myLine1] (encoder.east) to[out=0, in=180] (decoder.west);
        
        \draw[myLine1] (input.east) to[out=0, in=180] (lstm.west);
        \draw[myLine1] (lstm.east) to[out=0, in=180] (output.west);
      
     
      \node[below=1.7cm of input, inner sep=0, anchor=center] (input2) {$X$};
      \matrix[right=0.75cm of input2, row sep=0mm, column sep=2.5mm, inner sep=1mm, bigbox, every node/.style=box3](lstm2) {
            \node(embedding2){\footnotesize{\textbf{Embedding}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
            &  \node(encoder2){\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{LSTM} \nodepart{third} \scriptsize{Transformer}}; 
            & \node(decoder2){\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; \\
        };
        \node[inner sep=0, anchor=center, above=0.34cm of embedding2] (role) {$c$};
        \node[inner sep=0, anchor=center, above=0.3cm of encoder2] (concat) {$\oplus$};
        \node[inner sep=0, anchor=center, right=0.75cm of lstm2] (output2) {$\hat{Y}$};

        \draw[myLine1] (embedding2.east) to[out=0, in=180] (encoder2.west);
        \draw[myLine1] (encoder2.north) to[out=90, in=-90] (concat.south);
        \draw[myLine1] (concat.east) to[out=0, in=90] (decoder2.north);
        \draw[myLine1] (role.east) to[out=0, in=180] (concat.west);
        
        
        \draw[myLine1] (input2.east) to[out=0, in=180] (lstm2.west);
        \draw[myLine1] (lstm2.east) to[out=0, in=180] (output2.west);
      
      \end{tikzpicture}
\caption{Single-output unconditional (top) and conditional methods (bottom).}%The input state, $X$, is embedded with a MLP. Then, we 
%extract temporal features with LSTM (for RED and cRED models) or with a Transformer-based encoder (for TF and cTF models). Finally, the decoder takes as input 
%the temporal features and produces the future velocity vector, $\hat{Y}$. The conditional methods (right) concatenate the embedded agent class to 
%the temporal features and proceed to the decoding stage.}
\label{fig:sing_out_overview}
\end{figure}

\begin{figure}[!t]
  \centering
  \begin{tikzpicture}[
    >=Stealth,
    node distance=1.5cm,
    normalbox/.style={draw=black, rectangle, minimum width=0.8cm, minimum height=0.8cm, align=center},
    bigbox/.style = {draw=black, thick, fill=green!25, rounded corners, rectangle, minimum width = 4cm, minimum height = 4cm},
    box3/.style = {minimum size=0.2cm, rounded corners, draw=green!25, fill=blue!10},
    box2/.style = {minimum size=0.2cm, rounded corners, draw=green!25, fill=yellow!10},
    arrow/.style={->, thick, >=stealth},
]

  % Input embeddings
  % \node[inner sep=0, anchor=center] (input) at (-10,0.05) {\scriptsize{$X$}};
  % \node[normalbox, right=0.3cm of input] (mlp_emb) {\scriptsize{MLP}};
  % Positional encoding
  \node[inner sep=0, anchor=center] (input) at (-10,0.05) {\scriptsize{Embedded}};
  \node[below=0.0cm of input] (input2) {\scriptsize{$X$}};
  \node[normalbox, right=0.3cm of input] (pos1) {\scriptsize{Positional}\\\scriptsize{Encoding}};
  % Layer
  \draw[fill=green!10] (-7.7,0.75) -- (-7.7,-0.75) -- (-3.3,-0.75) -- (-3.3,0.75) -- cycle;

  \node[box2](mha)  at (-6.,0.4) {\scriptsize{MHA}};
  \node[box3, below=3mm of mha](plus) {\scriptsize{Add.}};
  \node[box2, left=4mm of mha](ln) {\scriptsize{LN}};
  \node[box3, right=1.5cm of plus](plus2) {\scriptsize{Add.}};
  \node[box2, right=5mm of mha](ln2) {\scriptsize{LN}};
  \node[box2, right=4mm of ln2](ffn) {\scriptsize{FFN}};
  \node[right=5.2cm of pos1] (tf) {\scriptsize{Temp.}};
  \node[below=0.0cm of tf] (tf2) {\scriptsize{Feat.}};

  % \draw[arrow] (input.east) to[out=0, in=180] (mlp_emb.west);
  \draw[arrow] (input.east) to[out=0, in=180] (pos1.west);
  
  \draw[arrow] (pos1.east) -- ++(0,0.35) -- (ln.west);
  \draw[arrow] (pos1.east) -- ++(0,-0.35) -- (plus.west);

  \draw[arrow] (plus.east) to[out=0, in=180] (plus2.west);
  \draw[arrow] (ln.east) to[out=0, in=180] (mha.west);
  \draw[arrow] (mha.south) to[out=270, in=90] (plus.north);
  \draw[arrow] (plus.east) -- ++(0,0) -- (ln2.west);
  \draw[arrow] (ln2.east) to[out=0, in=180] (ffn.west);
  \draw[arrow] (ffn.south) to[out=270, in=90] (plus2.north);
  \draw[arrow] (plus2.east) to[out=0, in=180] (tf.west);
  
  \end{tikzpicture}
    \caption{Transformer encoder system for temporal features extraction.}
    \label{fig:tf_mec}
\vspace*{-4mm}
\end{figure}




\subsubsection{GAN-based Trajectory Predictors}
%Inspired by~\cite*{almeida23, kothari23}, we compare novel configurations for multiple-output methods, i.e., GANs and VAEs. In this paper, we propose 
%to change the temporal feature extractors used in \cite{almeida23} to transformer-based methods as in~\cite{kothari23}. In~\cite{kothari23},
%the authors introduce the transformer architecture as the discriminator's feature extractor. In this paper, we go beyond the use of 
%a transformer as the discriminator's feature extractor, and propose also a transformer-based generator and a transformer-based VAE. 
%These changes reflect the more recent architectures that strengthen the sequence modeling as shown in~\cite{kothari23}.
%GAN-based trajectory predictors lie in the generative models' domain of trajectory prediction. 
%Comprising two concurrently operating networks ---  --- a 
A GAN aims to reconstruct 
the generative process of the underlying input data using two modules: generator ($G$) and discriminator ($D$). The generator maps the input state $X$ and a latent random vector $\mathbf{z_G}$, to a realistic future set of velocities, $Y$. 
We sample the latent vector from a standard normal Gaussian distribution. 
Simultaneously, the discriminator differentiates both real and generated future velocity vectors, $Y$ and 
$\hat{Y}$, respectively. Consequently, as the generator strives to deceive the discriminator with realistic samples, the 
latter refines its discrimination ability over time due to the escalating complexity of its task. This adversarial 
training scenario is essential for producing multiple plausible trajectories. %Notably, the distinction between a GAN and a conditional GAN (cGAN) lies in the latter considering the class of each trajectory, denoted as $c$. 
In the class-conditioned GAN (cGAN), both the generator and discriminator incorporate the trajectory class as an additional input.
We optimize the GAN and cGAN discriminators using the binary cross-entropy loss, while the GAN generator is optimized with 
a weighted sum given by:
\begin{equation}
      L_{G} 
      = 
      \lambda_1 L_{T} + \lambda_2 
      \left(\frac{1}{2} \mathbb{E}[(D(Y) - 1)^2] + \frac{1}{2} \mathbb{E}[D(\hat{Y})^2]\right),
\end{equation}
%
where $\lambda_1$ and $\lambda_2$  are the weights applied to the MSE term $L_{T}$ (Eq.~\ref{eq:l_traj}) and 
to the GAN loss, respectively. 
In the training of the conditional variant (cGAN), the class is additionally fed as input to both the generator and the discriminator.
%

\begin{comment}
Fig.~\ref{fig:gan_based} illustrates the network configurations for GAN and cGAN models. In general, the generator 
employs an MLP to embed the state input, $X$, followed by a transformer encoder-based network that encodes the embedded input state. 
This encoded representation is then concatenated with the latent vector, $\mathbf{z_G}$, and passed through a final MLP decoder, 
ultimately yielding the predicted velocity vector, $\hat{Y}$. Analogously to~\cite{kothari23}, the discriminator comprises a 
transformer-encoder network and an MLP in the final layer. For cGAN, both generator and discriminator, concatenate the embedding of the trajectory's class to their respective input. 
Therefore, the inputs of the cGAN network becomes: $s\oplus c$  for the generator and $Y\oplus c$ or $\hat{Y}\oplus c$ for the discriminator.  
\end{comment}

\cref{fig:gan_based} illustrates the network configurations for GAN and cGAN models. In general, the generators have the same layer configuration as the TF model. The difference is the latent vector, $\mathbf{z_G}$, which is concatenated with the temporal features from the transformer and passed to the decoder. Analogously to~\cite{kothari23}, the discriminator comprises a 
transformer-encoder network and an MLP in the final layer. For cGAN, both the generator and the discriminator concatenate $X$ to the embedding of the trajectory class ($c$). In the generator, $c$ is also concatenated to the input of the decoder. 
 
\begin{comment}
    
\begin{figure}[t]
  \centering
  \tikzset{myLine1/.style = {->, thick, >=stealth},
    mynarrownodes/.style = {node distance=0.75cm and 0.3cm},
    }
  \tikzstyle{gen_dashed} = [minimum width=2.4cm, minimum height=3.8cm, draw=black, dashed, rectangle]
  \tikzstyle{disc_dashed} = [minimum width=1.6cm, minimum height=3.8cm, draw=black, dashed, rectangle]
  \tikzstyle{bigbox} = [draw=black!50, thick, fill=gray!50, rounded corners, rectangle]
  \tikzstyle{box} = [minimum size=0.2cm, rounded corners,rectangle split,rectangle split parts=2, inner sep=0.1ex, fill=gray!10]
  \tikzstyle{box_decoder} = [minimum size=0.2cm, rounded corners,rectangle split,rectangle split parts=4, inner sep=0.1ex, fill=gray!10]
  \begin{subfigure}{0.48\columnwidth}
    \centering
      \begin{tikzpicture}
      \node[inner sep=0, anchor=center] (input) at (-4,2) {$X$};
      \node[style=gen_dashed, fill=yellow!5](gen_dash) at (-4.35,-0.25){}; 
      \node[inner sep=0, anchor=center] (g_str) at (-5.25,1.4) {$G$};
      \node[right=0.07cm of gen_dash, style=disc_dashed, fill=blue!5](disc_dash){}; 
      \node[inner sep=0, anchor=center] (d_str) at (-2.8,1.4) {$D$};
      

      
      \matrix[below=0.75cm of input, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](gen) {
            \node(embedding)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
            \\  \node(encoder)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; 
            \\ \node(decoder)[style=box]{\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; \\
        };
        \node[inner sep=0, anchor=center, below=1.1cm of gen] (output) {$\hat{Y}$};
        \node[inner sep=0, anchor=center, left=0.58cm of embedding] (noise) {$z_G$};
        \node[inner sep=0, anchor=center, left=0.55cm of encoder] (concat) {$\oplus$};
        

        \draw[myLine1] (embedding.south) to[out=-90, in=90] (encoder.north);
        \draw[myLine1] (encoder.west) to[out=180, in=0] (concat.east);
        \draw[myLine1] (noise.south) to[out=-90, in=90] (concat.north);
        \draw[myLine1] (concat.south) to[out=-90, in=180] (decoder.west);

        \node[inner sep=0, anchor=center, right=1cm of input] (inputd) {$Y$ or $\hat{Y}$};
        \matrix[below=1.5cm of inputd, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](disc) { 
          \node(class)[style=box_decoder]{\footnotesize{\textbf{Classifier}} \vphantom{$\vcenter{\vspace{1.em}}$}\nodepart{second} \scriptsize{Transformer} \nodepart{third} \scriptsize{+} \nodepart{fourth} \scriptsize{MLP}}; \\
        };
        \node[inner sep=0, anchor=center, below=1.7cm of disc] (score) {$s$};
        
        
        
        \draw[myLine1] (input.south) to[out=-90, in=90] (gen.north);
        \draw[myLine1] (gen.south) to[out=-90, in=90] (output.north);
        \draw[myLine1] (inputd.south) to[out=-90, in=90] (disc.north);
        \draw[myLine1] (disc.south) to[out=-90, in=90] (score.north);
      
      \end{tikzpicture}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.48\columnwidth}
    \centering
      \begin{tikzpicture}
      \node[inner sep=0, anchor=center] (input) at (-3.7,2) {$X \oplus c$};
      \node[style=gen_dashed, fill=yellow!15](gen_dash) at (-4.1,-0.25){}; 
      \node[inner sep=0, anchor=center] (g_str) at (-5.05,1.4) {$cG$};
      \node[right=0.13cm of gen_dash, style=disc_dashed, fill=blue!15](disc_dash){}; 
      \node[inner sep=0, anchor=center] (d_str) at (-2.5,1.4) {$cD$};
      

      
      \matrix[below=0.75cm of input, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](gen) {
            \node(embedding)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
            \\  \node(encoder)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; 
            \\ \node(decoder)[style=box]{\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} 
            \nodepart{second} \scriptsize{MLP}}; \\
        };
        \node[inner sep=0, anchor=center, below=1cm of gen] (output) {$\hat{Y}$};
        \node[inner sep=0, anchor=center, left=0.58cm of embedding] (noise) {$z_G$};
        \node[inner sep=0, anchor=center, left=0.55cm of encoder] (concat) {$\oplus$};
        
        \draw[myLine1] (embedding.south) to[out=-90, in=90] (encoder.north);
        \draw[myLine1] (encoder.west) to[out=180, in=0] (concat.east);
        \draw[myLine1] (noise.south) to[out=-90, in=90] (concat.north);
        \draw[myLine1] (concat.south) to[out=-90, in=180] (decoder.west);

        \node[inner sep=0, anchor=center, right=1.2cm of input] (inputd) {$c$};
        \node[inner sep=0, anchor=center, above=0.15mm of inputd] (cat) {$\oplus$};
        \node[inner sep=0, anchor=center, above=0.1mm of cat] (ys) {$Y$ or $\hat{Y}$};
        \matrix[below=1.5cm of inputd, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](disc) { 
          \node(class)[style=box_decoder]{\footnotesize{\textbf{Classifier}} \vphantom{$\vcenter{\vspace{1.em}}$}\nodepart{second} \scriptsize{Transformer} \nodepart{third} \scriptsize{+} \nodepart{fourth} \scriptsize{MLP}}; \\
        };
        \node[inner sep=0, anchor=center, below=1.7cm of disc] (score) {$s$};
        
        
        
        \draw[myLine1] (input.south) to[out=-90, in=90] (gen.north);
        \draw[myLine1] (gen.south) to[out=-90, in=90] (output.north);
        \draw[myLine1] (inputd.south) to[out=-90, in=90] (disc.north);
        \draw[myLine1] (disc.south) to[out=-90, in=90] (score.north);
      
      \end{tikzpicture}
  \end{subfigure}
  \caption{GAN-based models: unconditional GAN (left) and cGAN (right).}
  \label{fig:gan_based}
  \vspace*{-6mm}
\end{figure}
\end{comment}

\begin{figure}[t]
  \centering
  \tikzset{myLine1/.style = {->, thick, >=stealth},
    mynarrownodes/.style = {node distance=0.75cm and 0.3cm},
    }
  \tikzstyle{gen_dashed} = [minimum width=2.32cm, minimum height=3cm, draw=black, dashed, rectangle]
  \tikzstyle{disc_dashed} = [minimum width=1.55cm, minimum height=3cm, draw=black, dashed, rectangle]
  \tikzstyle{bigbox} = [draw=black!50, thick, fill=gray!50, rounded corners, rectangle]
  \tikzstyle{box} = [minimum size=0.2cm, rounded corners,rectangle split,rectangle split parts=2, inner sep=0.1ex, fill=gray!10]
  \tikzstyle{box_decoder} = [minimum size=0.2cm, rounded corners,rectangle split,rectangle split parts=4, inner sep=0.1ex, fill=gray!10]
  \begin{subfigure}{0.48\columnwidth}
    \centering
      \begin{tikzpicture}
      \node[inner sep=0, anchor=center] (input) at (-4,2) {$X$};
      \node[style=gen_dashed, fill=yellow!5,minimum width=2.1cm](gen_dash) at (-4.27,0.1){}; 
      \node[inner sep=0, anchor=center] (g_str) at (-5.1,1.4) {$G$};
      \node[right=0.06cm of gen_dash, style=disc_dashed, fill=blue!5](disc_dash){}; 
      \node[inner sep=0, anchor=center] (d_str) at (-2.95,1.4) {$D$};

\begin{comment}
    https://fs.aalto.fi/adfs/ls/?client-request-id=3c942044-7aa7-10b6-f1a3-49dffe6af823&username=&wa=wsignin1.0&wtrealm=urn%3afederation%3aMicrosoftOnline&wctx=estsredirect%3d2%26estsrequest%3drQQIARAAjZE9bBJhAIb5OHr2xx_SwcFFg05tDu4OuB-iA3BXoID8FCitMeR691057ue7cndQaDrrYtIYFzs42EHTyTgY08VuJp262sTYODWaGHXqZIS4uOkzvHmnd3ifOYwKU4lb5B9oYpwEqaoUIcNx-4vu7HRQuPHk9ovhm-CPvdynX53zm7tgUpIMF4VVbR9cb7uu7SQiEeS5BkJ6GKmqJsOwjMwI6kuRtwAcA3AGwL6fZaJcjGKYOMfSDBWlWYYNrylcXGYhTfAMGSNiqkwTHMtThCLFaEamJJVWoif-K6Wk57bpcaCuNoQ__VMq6potGznuLvYeCLLHCijXz4hCG3ktrWEaLbQIU17KKMpFsUDmaXKxKrYXc411mHVYNSOzYr2AMqlBWstV1oftfLXurAz6K9lqSuh04hyTH2aT2WUhvxTrVqLryeXmwoKnJDt36zydruULgx4sszZRyDvQqsfLTcMq88wqX7Msb0PL5SHjREsN06S7dqVsD3S7JG3qIu9siILTbfSbjSVFVXqm6xp2tkR6IrXcalW5fey_nLzG8NG7JrKOMBzZ0NKU4wA4DYAvAT85eR4AzydG0q4-27um8x-FdzPNz4ePPviOJiJti6z1CxWvPxIg69V2MSmnV4u1Db3XFzPGmh5R5uHmfIbzIHmHTVA7ONjB8QN8ahIL-kJYukyd4eA7Dh5e8B1M_Uv78Qw4uRibxmVD0kxndm4rpCktF-nQCiW2Qpum05LlcetJhgedUOJeaLQfur-9vX14yXd--eXX052njx98y74K-n4D0&RedirectToIdentityProvider=AD+AUTHORITY
\end{comment}
      
      \matrix[below=0.5cm of input, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](gen) {
            \node(embedding)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
            \\  \node(encoder)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; 
            \\ \node(decoder)[style=box]{\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; \\
        };
        \node[inner sep=0, anchor=center, below=0.6cm of gen] (output) {$\hat{Y}$};
        \node[inner sep=0, anchor=center, left=0.34cm of embedding] (noise) {$z_G$};
        \node[inner sep=0, anchor=center, left=0.3cm of encoder] (concat) {$\oplus$};
        

        \draw[myLine1] (embedding.south) to[out=-90, in=90] (encoder.north);
        \draw[myLine1] (encoder.west) to[out=180, in=0] (concat.east);
        \draw[myLine1] (noise.south) to[out=-90, in=90] (concat.north);
        \draw[myLine1] (concat.south) to[out=-90, in=180] (decoder.west);

        \node[inner sep=0, anchor=center, right=0.9cm of input] (inputd) {$Y$ or $\hat{Y}$};
        \matrix[below=1.25cm of inputd, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](disc) { 
          \node(class)[style=box_decoder]{\footnotesize{\textbf{Classifier}} \vphantom{$\vcenter{\vspace{1.em}}$}\nodepart{second} \scriptsize{Transformer} \nodepart{third} \scriptsize{+} \nodepart{fourth} \scriptsize{MLP}}; \\
        };
        \node[inner sep=0, anchor=center, below=1.2cm of disc] (score) {$s$};
        
        
        
        \draw[myLine1] (input.south) to[out=-90, in=90] (gen.north);
        \draw[myLine1] (gen.south) to[out=-90, in=90] (output.north);
        \draw[myLine1] (inputd.south) to[out=-90, in=90] (disc.north);
        \draw[myLine1] (disc.south) to[out=-90, in=90] (score.north);
      
      \end{tikzpicture}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.48\columnwidth}
    \centering
      \begin{tikzpicture}
      \node[inner sep=0, anchor=center] (input) at (-3.7,2) {$\ccircled{$c$}\oplus X$};
      \node[style=gen_dashed, fill=yellow!15](gen_dash) at (-4.1,0.1){}; 
      \node[inner sep=0, anchor=center] (g_str) at (-4.96,1.4) {$cG$};
      \node[right=0.04cm of gen_dash, style=disc_dashed, fill=blue!15](disc_dash){}; 
      \node[inner sep=0, anchor=center] (d_str) at (-2.5,1.4) {$cD$};
      

      
      \matrix[below=0.5cm of input, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](gen) {
            \node(embedding)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
            \\  \node(encoder)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; 
            \\ \node(decoder)[style=box]{\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} 
            \nodepart{second} \scriptsize{MLP}}; \\
        };
        \node[inner sep=0, anchor=center, below=0.6cm of gen] (output) {$\hat{Y}$};
        \node[inner sep=0, anchor=center, left=0.34cm of embedding] (noise) {$z_G$};
        \node[inner sep=0, anchor=center, left=0.3cm of encoder] (concat) {$\oplus$};
        
        \draw[myLine1] (embedding.south) to[out=-90, in=90] (encoder.north);
        \draw[myLine1] (encoder.west) to[out=180, in=0] (concat.east);
        \draw[myLine1] (noise.south) to[out=-90, in=90] (concat.north);
        \draw[myLine1] (concat.south) to[out=-90, in=180] (decoder.west);

        \node[inner sep=0, anchor=center, right=0.95cm of input] (inputd) {$c$};
        \node[inner sep=0, anchor=center, above=0.15mm of inputd] (cat) {$\oplus$};
        \node[inner sep=0, anchor=center, above=0.1mm of cat] (ys) {$Y$ or $\hat{Y}$};
        \matrix[below=1.25cm of inputd, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](disc) { 
          \node(class)[style=box_decoder]{\footnotesize{\textbf{Classifier}} \vphantom{$\vcenter{\vspace{1.em}}$}\nodepart{second} \scriptsize{Transformer} \nodepart{third} \scriptsize{+} \nodepart{fourth} \scriptsize{MLP}}; \\
        };
        \node[inner sep=0, anchor=center, below=1.2cm of disc] (score) {$s$};
        \draw[myLine1] (input.west) -| (-5.2, 0.5) |- (concat.west);
        
        
        
        \draw[myLine1] (input.south) to[out=-90, in=90] (gen.north);
        \draw[myLine1] (gen.south) to[out=-90, in=90] (output.north);
        \draw[myLine1] (inputd.south) to[out=-90, in=90] (disc.north);
        \draw[myLine1] (disc.south) to[out=-90, in=90] (score.north);
      
      \end{tikzpicture}
  \end{subfigure}
  \caption{GAN-based models: unconditional GAN (left) and cGAN (right).}
  \label{fig:gan_based}
  \vspace*{-2mm}
\end{figure}



\subsubsection{VAE-based Trajectory Predictors}

Also categorized as generative models, VAE-based predictors involve two integral networks: the prior network $p_\theta$ and the recognition network $q_\phi$. The prior network captures the mapping from the input state $X$ and a latent vector $\mathbf{z_V}$ to the predicted 
trajectory $Y$. In parallel, the recognition network learns to map the ground truth trajectory $Y$, to the parameters 
of a Gaussian distribution, effectively representing a lower-dimensional latent space. We adopt 
a standard normal Gaussian as the prior for the underlying distribution of future trajectories. The Kullback-Leibler (KL) divergence is then employed to approximate the learned distribution to the prior, therefore,  the VAE's loss function 
is given by:
%
\begin{equation}
      L_{V} = \beta_1 ~ L_T 
      - \beta_2 ~ D_\mathrm{KL}[q_{\phi}(z_V | Y) \rVert p_{\theta}(z_V | X)], 
  \end{equation}
  %
  where $\beta_1$ and $\beta_2$ are the weights applied to the MSE and KL terms, respectively. In the training of the conditional variant (cVAE), the class
  of the agent's trajectory is added as input to both the predictor and recognition networks.
  %

\begin{comment}  
  Fig.~\ref{fig:vae_based} depicts the network configurations for VAE and cVAE models.
  Analogous to the generator in a GAN, the prior network initiates the process by embedding the input state using a 
  MLP. Subsequently, a transformer-encoder network processes the sequence of embedded positions, 
  and the resultant encoded features are concatenated with the latent vector $\mathbf{z_V}$. This concatenated vector 
  undergoes decoding through an MLP network yielding the predicted velocity vector.
  Simultaneously, the recognition network follows a comparable procedure, with the decoding process generating two 
  parameters representing the learned Gaussian parameters. Also, similarly to cGAN, cVAE networks concatenate the respective inputs to the trajectory's class.
\end{comment}

\cref{fig:vae_based} shows the network configurations for the VAE and cVAE models. The predictor's network configuration  is identical to the generator in the GAN and cGAN models. The difference lies in the training process, where the latent vector, $\mathbf{z_V}$, is sampled based on parameters generated by the recognition network ($q_\phi$). The recognition network processes the ground truth prediction akin to 
$p_\theta$, but concludes with two linear layers producing the Gaussian parameters.

\begin{comment}
    
  \begin{figure}[t]
    \centering
    \tikzset{myLine1/.style = {->, thick, >=stealth},
      mynarrownodes/.style = {node distance=0.75cm and 0.3cm},
      }
    \tikzstyle{q_dashed} = [minimum width=1.65cm, minimum height=4cm, draw=black, dashed, rectangle]
    \tikzstyle{bigbox} = [draw=black!50, thick, fill=gray!50, rounded corners, rectangle]
    \tikzstyle{box} = [minimum size=0.2cm, rounded corners,rectangle split,rectangle split parts=2, inner sep=0.1ex, fill=gray!10]
    \tikzstyle{box_decoder} = [minimum size=0.2cm, rounded corners,rectangle split,rectangle split parts=4, inner sep=0.1ex, fill=gray!10]
    \begin{subfigure}{0.48\columnwidth}
      \centering
        \begin{tikzpicture}
        \node[inner sep=0, anchor=center] (input) at (-6,2) {$X$};
        \node[style=q_dashed, fill=white](q_dash) at (-4.0,-0.25){}; 
        \node[inner sep=0, anchor=center] (q_str) at (-3.4,1.4) {$q_{\phi}$};
        \node[inner sep=0, anchor=center] (q_str) at (-5.7,1.4) {$p_\theta$};
  
        \matrix[below=0.75cm of input, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](vae) {
              \node(embedding1)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
              \\  \node(encoder)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; 
              \\ \node(decoder)[style=box]{\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} 
              \nodepart{second} \scriptsize{MLP}}; \\
          };
          \node[inner sep=0, anchor=center, below=0.75cm of vae] (output) {$\hat{Y}$};
          
          \draw[myLine1] (embedding1.south) to[out=-90, in=90] (encoder.north);
          \draw[myLine1] (input.south) to[out=-90, in=90] (vae.north);
          \draw[myLine1] (vae.south) to[out=-90, in=90] (output.north);
  
          \node[inner sep=0, anchor=center, right=1.7cm of input] (inputr) {$Y$};
          \matrix[below=0.75cm of inputr, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](recog) {
              \node(embedding_r)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
              \\  \node(encoder_r)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; 
              \\ \node(out_r)[style=box]{\footnotesize{\textbf{Output}} \vphantom{$\vcenter{\vspace{1.em}}$} 
              \nodepart{second} \scriptsize{Linear}}; \\
          };
  
          \node[inner sep=0, anchor=center, below=0.6cm of out_r] (noise) {$\hat{z_V}$};
          \node[inner sep=0, anchor=center, right=0.28cm of decoder] (concat) {$\oplus$};
          \draw[myLine1] (embedding_r.south) to[out=-90, in=90] (encoder_r.north);
          \draw[myLine1] (inputr.south) to[out=-90, in=90] (recog.north);
          \draw[myLine1] (recog.south) to[out=-90, in=90] (noise.north);
          \draw[myLine1] (noise.west) to[out=-180, in=-90] (concat.south);
          \draw[myLine1] (encoder.east) to[out=0, in=90] (concat.north);
          \draw[myLine1] (concat.west) to[out=-180, in=0] (decoder.east);
          \draw[myLine1] (encoder_r.south) to[out=270, in=90] (out_r.north);
  
          
        
        \end{tikzpicture}
    \end{subfigure}
    \hfill
      \begin{subfigure}{0.48\columnwidth}
      \centering
        \begin{tikzpicture}
        \node[inner sep=0, anchor=center] (input) at (-6,2) {$X \oplus c$};
        \node[style=q_dashed, fill=white](q_dash) at (-3.9,-0.25){}; 
        \node[inner sep=0, anchor=center] (q_str) at (-3.3,1.4) {$q_{\phi}$};
        \node[inner sep=0, anchor=center] (q_str) at (-5.7,1.4) {$p_\theta$};
  
        \matrix[below=0.75cm of input, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](vae) {
              \node(embedding1)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
              \\  \node(encoder)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; 
              \\ \node(decoder)[style=box]{\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} 
              \nodepart{second} \scriptsize{MLP}}; \\
          };
          \node[inner sep=0, anchor=center, below=0.75cm of vae] (output) {$\hat{Y}$};
          
          \draw[myLine1] (embedding1.south) to[out=-90, in=90] (encoder.north);
          \draw[myLine1] (input.south) to[out=-90, in=90] (vae.north);
          \draw[myLine1] (vae.south) to[out=-90, in=90] (output.north);
  
          \node[inner sep=0, anchor=center, right=1.2cm of input] (inputr) {$Y\oplus c$};
          \matrix[below=0.75cm of inputr, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](recog) {
              \node(embedding_r)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
              \\  \node(encoder_r)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; 
              \\ \node(out_r)[style=box]{\footnotesize{\textbf{Output}} \vphantom{$\vcenter{\vspace{1.em}}$} 
              \nodepart{second} \scriptsize{Linear}}; \\
          };
  
          \node[inner sep=0, anchor=center, below=0.6cm of out_r] (noise) {$\hat{z_V}$};
          \node[inner sep=0, anchor=center, right=0.21cm of decoder] (concat) {$\oplus$};
          \draw[myLine1] (embedding_r.south) to[out=-90, in=90] (encoder_r.north);
          \draw[myLine1] (inputr.south) to[out=-90, in=90] (recog.north);
          \draw[myLine1] (recog.south) to[out=-90, in=90] (noise.north);
          \draw[myLine1] (noise.west) to[out=-180, in=-90] (concat.south);
          \draw[myLine1] (encoder.east) to[out=0, in=90] (concat.north);
          \draw[myLine1] (concat.west) to[out=-180, in=0] (decoder.east);
          \draw[myLine1] (encoder_r.south) to[out=270, in=90] (out_r.north);
  
          
        
        \end{tikzpicture}
    \end{subfigure}
  \caption{VAE-based models: unconditional VAE (left) and cVAE (right). The recognition network ($q_{\phi}$, enclosed with dashed border) is 
  solely available during training.}
  \label{fig:vae_based}
  \vspace*{-6mm}
  \end{figure}
\end{comment}

  \begin{figure}[t]
    \centering
    \tikzset{myLine1/.style = {->, thick, >=stealth},
      mynarrownodes/.style = {node distance=0.75cm and 0.3cm},
      }
    \tikzstyle{q_dashed} = [minimum width=1.65cm, minimum height=3cm, draw=black, dashed, rectangle]
    \tikzstyle{bigbox} = [draw=black!50, thick, fill=gray!50, rounded corners, rectangle]
    \tikzstyle{box} = [minimum size=0.2cm, rounded corners,rectangle split,rectangle split parts=2, inner sep=0.1ex, fill=gray!10]
    \tikzstyle{box_dec} = [minimum size=0.2cm, rounded corners,rectangle split,rectangle split parts=2, inner sep=0.1ex, fill=gray!30, draw=gray!30]
    \begin{subfigure}{0.48\columnwidth}
      \centering
        \begin{tikzpicture}
        \node[inner sep=0, anchor=center] (input) at (-6,2) {$X$};
        \node[style=q_dashed, fill=white](q_dash) at (-4.0,0.25){}; 
        \node[inner sep=0, anchor=center] (q_str) at (-3.4,1.6) {$q_{\phi}$};
        \node[inner sep=0, anchor=center] (q_str) at (-5.7,1.6) {$p_\theta$};
  
        \matrix[below=0.5cm of input, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](vae) {
              \node(embedding1)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
              \\  \node(encoder)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; \\
              %\\ \node(decoder)[style=box]{\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} 
              %\nodepart{second} \scriptsize{MLP}}; \\
          };
          \node(decoder)[below=0.3cm of vae,style=box_dec]{\footnotesize{\textbf{Decoder}}\nodepart{second} \scriptsize{MLP}};

          
          \node[inner sep=0, anchor=center, below=0.5cm of decoder] (output) {$\hat{Y}$};
          
          \draw[myLine1] (embedding1.south) to[out=-90, in=90] (encoder.north);
          \draw[myLine1] (input.south) to[out=-90, in=90] (vae.north);
          \draw[myLine1] (decoder.south) to[out=-90, in=90] (output.north);
  
          \node[inner sep=0, anchor=center, right=1.7cm of input] (inputr) {$Y$};
          \matrix[below=0.5cm of inputr, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](recog) {
              \node(embedding_r)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
              \\  \node(encoder_r)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; 
              \\ \node(out_r)[style=box]{\footnotesize{\textbf{Output}} \vphantom{$\vcenter{\vspace{1.em}}$} 
              \nodepart{second} \scriptsize{Linear}}; \\
          };
  
          \node[inner sep=0, anchor=center, below=0.6cm of out_r] (noise) {$\hat{z_V}$};
          \node[inner sep=0, anchor=center, right=0.28cm of decoder] (concat) {$\oplus$};
          \draw[myLine1] (embedding_r.south) to[out=-90, in=90] (encoder_r.north);
          \draw[myLine1] (inputr.south) to[out=-90, in=90] (recog.north);
          \draw[myLine1] (recog.south) to[out=-90, in=90] (noise.north);
          \draw[myLine1] (noise.west) to[out=-180, in=-90] (concat.south);
          \draw[myLine1] (encoder.east) to[out=0, in=90] (concat.north);
          \draw[myLine1] (concat.west) to[out=-180, in=0] (decoder.east);
          \draw[myLine1] (encoder_r.south) to[out=270, in=90] (out_r.north);
  
          
        
        \end{tikzpicture}
    \end{subfigure}
    \hfill
      \begin{subfigure}{0.48\columnwidth}
      \centering
        \begin{tikzpicture}
        \node[inner sep=0, anchor=center] (input) at (-6,2) {$X\oplus$ \ccircled{$c$}};
        \node[style=q_dashed, fill=white](q_dash) at (-3.82,0.25){}; 
        \node[inner sep=0, anchor=center] (q_str) at (-3.3,1.6) {$q_{\phi}$};
        \node[inner sep=0, anchor=center] (q_str) at (-5.7,1.6) {$p_\theta$};
  
        \matrix[below=0.5cm of input, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](vae) {
              \node(embedding1)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
              \\  \node(encoder)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; \\
              %\\ \node(decoder)[style=box]{\footnotesize{\textbf{Decoder}} \vphantom{$\vcenter{\vspace{1.em}}$} 
              %\nodepart{second} \scriptsize{MLP}}; \\
          };
          \node(decoder)[below=0.3cm of vae,style=box_dec]{\footnotesize{\textbf{Decoder}}\nodepart{second} \scriptsize{MLP}};
          
          \node[inner sep=0, anchor=center, below=0.5cm of decoder] (output) {$\hat{Y}$};
          
          \draw[myLine1] (embedding1.south) to[out=-90, in=90] (encoder.north);
          \draw[myLine1] (input.south) to[out=-90, in=90] (vae.north);
          \draw[myLine1] (decoder.south) to[out=-90, in=90] (output.north);
          
         
  
          \node[inner sep=0, anchor=center, right=1.2cm of input] (inputr) {$Y\oplus c$};
          \matrix[below=0.5cm of inputr, row sep=2.5mm, column sep=0mm, inner sep=1mm, bigbox](recog) {
              \node(embedding_r)[style=box]{\footnotesize{\textbf{Embed.}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{MLP}}; 
              \\  \node(encoder_r)[style=box]{\footnotesize{\textbf{Encoder}} \vphantom{$\vcenter{\vspace{1.em}}$} \nodepart{second} \scriptsize{Transformer}}; 
              \\ \node(out_r)[style=box]{\footnotesize{\textbf{Output}} \vphantom{$\vcenter{\vspace{1.em}}$} 
              \nodepart{second} \scriptsize{Linear}}; \\
          };
  
          \node[inner sep=0, anchor=center, below=0.6cm of out_r] (noise) {$\hat{z_V}$};
          \node[inner sep=0, anchor=center, right=0.21cm of decoder] (concat) {$\oplus$};
          \draw[myLine1] (input.east) -| (-4.78, 0) |- (concat.east);
          \draw[myLine1] (embedding_r.south) to[out=-90, in=90] (encoder_r.north);
          \draw[myLine1] (inputr.south) to[out=-90, in=90] (recog.north);
          \draw[myLine1] (recog.south) to[out=-90, in=90] (noise.north);
          \draw[myLine1] (noise.west) to[out=-180, in=-90] (concat.south);
          \draw[myLine1] (encoder.east) to[out=0, in=90] (concat.north);
          \draw[myLine1] (concat.west) to[out=-180, in=0] (decoder.east);
          \draw[myLine1] (encoder_r.south) to[out=270, in=90] (out_r.north);
  
          
        
        \end{tikzpicture}
    \end{subfigure}
  \caption{VAE-based models: unconditional VAE (left) and cVAE (right). The recognition network ($q_{\phi}$, enclosed with dashed border) is 
  solely available during training.}
  \label{fig:vae_based}
  \vspace*{-6mm}
  \end{figure}



\subsection{Pattern-based Trajectory Predictors}
Maps of Dynamics encode spatial or spatio-temporal motion patterns as a feature of the environment~\cite{kucner2017enabling, tomasz_survey23}. By generalizing velocity observations, human dynamics can be represented through flow models. Prior work proposes CLiFF-LHMP~\cite{zhu2023clifflhmp}, which exploits MoDs for long-term human motion prediction. It uses a multi-modal probabilistic representation of a velocity field (CLiFF-map), which is built from observations of human motion and employs Semi-Wrapped Gaussian mixture models (SWGMM) to capture the local distribution of velocities. %In the prediction process, the approach samples directions from the CLiFF-map at each predicted location and uses a Gaussian kernel function to bias a constant velocity prediction with the sampled direction. 
With the learned motion patterns, the predictor implicitly accounts for the obstacle layouts and predicts trajectories that follow the complex topology of the environment. CLiFF-LHMP has been shown to perform well for prediction horizons up to \SI{50}{\second} \cite{zhu2023clifflhmp} and with sparse, incomplete and very limited training data \cite{zhu2023data}.

In the CLiFF-LHMP method, a single CLiFF-map is employed for all predicted trajectories, irrespective of the agent class. However, motion patterns can vary depending on the class of the agent, as we show in Fig.~\ref{fig:CLiFF-mapSDD}. A zoomed-in view of example locations is shown in Fig.~\ref{fig:point-example-sdd}. Both direction and speed differ between {\em Bicyclist} and {\em Pedestrian}. In this work, we introduce a new variation of CLiFF-maps, namely class-conditioned CLiFF-map, which differentiates the motion patterns associated with various classes. 

In a class-conditioned CLiFF-map, individual CLiFF-maps $\Xi_c$ are built for each class of agents using their specific trajectories. For an agent with class $c$, we estimate $\mathcal{T}$ by sampling a velocity from $\Xi_c$ within the sampling radius $r_s$ for each prediction time step $t$. Then we estimate the new velocity using a biased version of the Constant Velocity Model (CVM). The estimation process is the same as that of CLiFF-LHMP, which is briefly described in the following. Please see \cite{zhu2023clifflhmp} for more details. The velocity prediction at time step $t$ is updated by biasing the last time step velocity with the sampled one as: $ \rho_t = \rho_{t-1} + (\rho_s - \rho_{t-1}) \cdot Kn(\rho_{s} - \rho_{t-1}), 
\theta_t = \theta_{t-1} + (\theta_s - \theta_{t-1}) \cdot Kn(\theta_{s} - \theta_{t-1})$, where $\rho$ and $\theta$ represent speed and heading orientation of the agent, respectively. The kernel function $Kn$, defined as $Kn(x) =  e ^ {-\beta \left\Vert x \right\Vert ^ 2}$, modulates the influence of the sampled velocity. Using kernel $Kn$, the MoD term is scaled by the deviation between sampled and current velocities according to the CVM. The MoD is trusted less if it deviates more from the current velocity. Parameter $\beta$ controls the reliance on the MoD versus the CVM, with a lower $\beta$ favoring the velocity sampled from the MoD.

%\begin{equation}
%\begin{gathered}
%\rho_t = \rho_{t-1} + (\rho_s - \rho_{t-1}) \cdot K(\rho_{s} - \rho_{t-1}), \\
%\theta_t = \theta_{t-1} + (\theta_s - \theta_{t-1}) \cdot K(\theta_{s} - \theta_{t-1}), \\
%\end{gathered}
%\end{equation}

\begin{figure}
\centering
\includegraphics[clip,trim=0mm 0mm 0mm 0mm,height=29mm]{figures/compare-mods/deathCircle_0.pdf}
\includegraphics[clip,trim=0mm 0mm 0mm 0mm,height=29mm]{figures/compare-mods/deathCircle_0_Biker.pdf}
\includegraphics[clip,trim=0mm 0mm 0mm 0mm,height=29mm]{figures/compare-mods/deathCircle_0_Pedestrian.pdf}%
\includegraphics[clip,trim=195mm 15mm 2mm 12mm,height=29mm]{figures/compare-mods/magni/colorbar.pdf}
\caption{General and class-conditioned CLiFF-maps in the {\em DeathCircle} scene of the SDD dataset ~\cite{robicquet16}. \textbf{Left:} combination of all classes, \textbf{middle:} {\em Bicyclist} class, \textbf{right:} {\em Pedestrian} class. The colored arrows show the mean value of each component in the SWGMM of CLiFF-map, which represents speed (arrow length) and orientation (arrow direction) jointly with a multimodal distribution. The motion patterns represented in CLiFF-maps exhibit distinct characteristics across different classes.}
\label{fig:CLiFF-mapSDD}
\vspace*{-4mm}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics*[width=0.9\linewidth]{figures/compare-mods/threedotindeathcircle_v3.pdf}
    \caption{CLiFF-maps at example locations in SDD ~\cite{robicquet16}. Both general and class-conditioned CLiFF-maps of {\em Bicyclist} and {\em Pedestrian} of three locations are shown on the \textbf{right}. General CLiFF maps may depict combinations of multiple classes (point 1) or median speed and orientation (points 2 and 3).}
\label{fig:point-example-sdd}
\vspace*{-6mm}
\end{figure}

==> contents/4_experiments.tex <==
\section{EXPERIMENTS} \label{section-experiments}
%This section describes the experiments conducted to showcase the impact of the semantic attributes present on the accuracy of trajectory prediction. We begin by outlining the experimental setup, including data preprocessing and analysis. We then describe the implementation details of the quantitative and qualitative experiments, along with the evaluation metrics used to assess predictors performance. 

\subsection{Datasets}
%We use two datasets for evaluation: the TH\"{O}R-MAGNI dataset and the Stanford Drone Dataset (SDD).
In this study, we evaluate and compare the performance of the trajectory prediction methods described in \cref{section-methods} on two datasets, TH\"{O}R-MAGNI and SDD. %These datasets represent distinct environments, with SDD situated in an outdoor university campus and TH\"{O}R-MAGNI in an indoor setting. Both datasets contain various classes of agents: TH\"{O}R-MAGNI comprises human-centred agents in an industrial environment whereas SDD includes road agents.
Importantly for our analysis, there is a substantial difference in class proportions between the two datasets. %, as illustrated in Fig.~\ref{fig:label_dist}.
Specifically, SDD shows a noticeable class imbalance compared to TH\"{O}R-MAGNI. This inter-dataset class imbalance constitutes a significant characteristic that is analyzed to assess its impact on the performance of the two categories of predictors under consideration: deep learning models and MoDs approaches.



%\noindent
\textbf{TH\"{O}R-MAGNI}: %This dataset~\cite{schreiter2022magni} is an extension of TH\"{O}R~\cite{rudenko2020thor}, which applies the TH\"{O}R data collection process with enriched and heterogeneous semantic attributes of human agents. TH\"{O}R-MAGNI is collected in a weakly-controlled laboratory environment using motion capture%\footnote{\url{www.qualisys.com}}
%to track the head position and orientation of every participant. 
TH\"{O}R-MAGNI contains 3.5 hours of human motion data in a laboratory setting where humans navigate and interact with static and mobile robots. 
In two of the five recorded scenarios (Scenarios 2 and 3), humans engage in activities modelled after industrial tasks, such as group or individual movement, transportation of various objects (e.g., boxes, buckets, and larger items like a poster stand, etc). These activities affect the motion patterns of the humans, namely in the velocity profile~\cite{almeida23}.
Therefore, in this paper, we focus on Scenarios 2, 3A and 3B of the dataset, where roles and tasks were assigned to the participants. These specific scenarios include 30 participants and entail a total motion duration of 1.5 hours. Five distinct agent roles were observed across all scenarios: {\em Carrier--Large Object}, {\em Visitors--Group}, {\em Visitors--Alone}, {\em Carrier--Bucket}, and {\em Carrier--Box}, with corresponding sample proportions of 25.7\%, 23.6\%, 22.7\%, 14.1\%, and 13.9\%.

%\noindent
\textbf{SDD}: %Stanford Drone Dataset~\cite{robicquet16} consists of multiple unique scenes captured on the Stanford university campus from a top-down view using a flying drone. The dataset contains various types of agents that navigate in a real-world outdoor environment. In total, SDD provides 60 videos and 6 annotated classes of agents.
SDD encompasses 5 hours of heterogeneous trajectory data captured across 60 videos on the Stanford University campus. 
It includes trajectories of bicyclists, pedestrians, skateboarders, carts, cars, and buses. 
Notably, certain classes, like {\em Bicyclist} and {\em Pedestrian}, coexist in shared spaces but exhibit distinct movement patterns, 
with bicyclists typically moving at a faster pace.
In SDD, the coordinates of agents are given in pixel values. For evaluating class-conditioned prediction methods, we choose the videos that contain at least two classes of agents and include more than 10 trajectories for each class, resulting in 7 scenes (gates, little, nexus, coupa, bookstore, deathCircle, hyang) with 3 classes of agents: {\em Pedestrian}, {\em Bicyclist} and {\em Car} with a corresponding sample proportions of 64.6\%, 34.3\%, and 1.1\%.


\subsection{Implementation Details}
To evaluate the predictors, we employed a repeated random sub-sampling validation method. %For each iteration, we randomly selected 10\% of the dataset for testing and used the remaining 90\% for training. 
For each iteration, we randomly selected $p\%$ of the dataset for training and used the remaining $(100-p)\%$ for testing. This process was repeated ten times, with the selection of test and training data being independently randomized in each iteration. %In the data efficiency analysis, we decreased the percentage of data used for training, from 90\% to 10\% in steps of 10\%. %For each training percentage, we randomly selected the corresponding proportion of the dataset for training, with the remainder for testing.
In the accuracy analysis (\cref{sec:acc}), we set $p=90$. In the data efficiency analysis (\cref{sec:data_eff}), we decreased the percentage of data used for training from $p=90$ to $p=10$ in steps of $10$.

Following current trajectory prediction benchmarks~\cite{Kothari2020HumanTF}, %for the experiments with both TH\"{O}R-MAGNI and SDD datasets, 
we take the past 8 time steps of the trajectory as observation ($O_p = 8$) and predict for the next 12 time steps ($T_p = 12$).


%%% Want to replace it with a table maybe? 
%\begin{figure}[!t]
%    \centering
%    \includegraphics*[width=.8\linewidth]{figures/label_dist.pdf}
%    \caption{Agents classes proportion across SDD and TH\"{O}R-MAGNI datasets. "P", "B" and "C" abbreviates {\em Pedestrian}, {\em Biker} and {\em Car}, respectively. "CBo", "CBu", "VA", "VG" and "CLO" abbreviates {\em Carrier--Box}, {\em Carrier--Bucket}, {\em Visitors--Alone}, {\em Visitors--Group} and {\em Carrier--Large Object}, respectively.} 
%    \label{fig:label_dist}
%\end{figure}

\begin{comment}
\begin{table}[!t]
    \centering
    \caption{Agents classes proportion.}
    \label{tab:t2_class_distribution}

    %\resizebox{\linewidth}{!}{
        \begin{tabular}{@{}c|c|c@{}}
        \toprule
        \textbf{\begin{tabular}[c]{@{}c@{}}Dataset\end{tabular}} &
            \textbf{Class} &
            \textbf{Portion (\%)} \\ \midrule
        \multirow{5}{*}{{MAGNI-S2}} &
            \begin{tabular}[c]{@{}c@{}}\emph{Carrier-Box}\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}13.9\end{tabular}
            \\ \cmidrule(l){2-3}
            &
            \emph{Carrier-Bucket} &
            \begin{tabular}[c]{@{}c@{}}14.1\end{tabular} 
            \\ \cmidrule(l){2-3}
            &
            \emph{Carrier-LO} &
            \begin{tabular}[c]{@{}c@{}}25.7\end{tabular}
            \\ \cmidrule(l){2-3}
            &
            \emph{Visitors-Alone} &
            \begin{tabular}[c]{@{}c@{}}22.7\end{tabular}  
            \\ \cmidrule(l){2-3}
            &
            \emph{Visitors-Group} &
            \begin{tabular}[c]{@{}c@{}}23.6\end{tabular}  
            
            \\ \specialrule{.2em}{.1em}{.1em}
        \multirow{2}{*}{{SDD}} &
            \emph{Pedestrian} &
            \begin{tabular}[c]{@{}c@{}}64.6\end{tabular} \\ \cmidrule(l){2-3} 
            &
            \emph{Bicyclist} &
            \begin{tabular}[c]{@{}c@{}}34.3\end{tabular} \\
            \cmidrule(l){2-3} 
            &
            \emph{Car} &
            \begin{tabular}[c]{@{}c@{}}1.1\end{tabular} \\ \bottomrule
        \end{tabular}%
   % }
\end{table}
\end{comment}

%\noindent
\textbf{For deep learning-based predictors}: 
We maintained a uniform hyperparameter setting across the deep learning models to ensure a fair 
comparison. The training process for all networks extended to a maximum of $100$ epochs 
with early stopping after $20$ epochs with no improvement. We optimize the networks 
with the Adam optimizer~\cite{adam_15_optim}, a learning 
rate of $1\mathrm{e}{-3}$ and a batch size of $32$. We also reduce the learning rate on the plateau of the validation loss during training (patience set to $5$ epochs).

For training generative models, including GAN, cGAN, VAE, and cVAE, we have standardized the weights in their 
respective loss functions. Consequently, $\lambda_1 = \beta_1 = 2$ and $\lambda_2 = \beta_2 = 1$, indicating a 
preference for the reconstruction of predictions based on the MSE term in the loss functions.

Finally, each model receives as input state the position concatenated with the velocity vector for TH\"{O}R-MAGNI scenarios. In contrast, for SDD, the velocity vector alone is used as input due to the aggregation of diverse scenes, making the position an irrelevant input feature.


%\noindent
\textbf{For MoD-based predictors}:
%For MoD-based predictors, CLiFF-LHMP~\cite{zhu2023clifflhmp} is evaluated in the experiments.
Identical parameters are used for both the class-conditioned CLiFF-LHMP and the general CLiFF-LHMP. The CLiFF-map grid resolutions for the SDD dataset and the TH\"{O}R-MAGNI dataset are 20 pixels and \SI{0.2}{\metre}, respectively. The sampling radius $r_s$ is aligned with the respective CLiFF-map grid resolution for each dataset. The kernel parameter is set to 5 across all experiments. In the figures and tables presenting results, CLiFF-LHMP is denoted as MoD and class-conditioned CLiFF-LHMP is referred as cMoD.

\subsection{Evaluation Metrics}
%TODO: FIX this section 
To compare the trajectory predictors, we use 
the \emph{Top-$K$ Average and Final Displacement Errors} (Top-$K$ ADE and FDE, in pixels for SDD and in meters for TH\"{O}R-MAGNI), 
as in~\cite{salzmann20,kothari23}. Top-$K$ ADE measures the  average $\ell_2$ distance between the ground truth track and the closest prediction (out of $K$ samples), and FDE measures the $\ell_2$ distance between the last position of the ground truth and the corresponding prediction. 
For evaluation, we present the results of Top-$1$ and Top-$3$ ADE/FDE. When $K=1$, we use the most likely output trajectory. 
We measure the mean and standard deviation of these metrics across iterations in the validation. 


%Finally, besides the models described in Section~\ref{section-methods}, we also report the metrics obtained by the 
%Constant Velocity Model (CVM)~\cite{scholler20}.




==> contents/5_results.tex <==
\section{RESULTS} \label{section-results}




\begin{table*}[!t]
    \centering
    \caption{Top-$1$ ADE/FDE scores (ADE on top of each row, FDE below) in TH\"{O}R-MAGNI Scenario 2 and SDD datasets in the 90\% train ratio setting. Bold values indicate the best performance comparing conditional models to their
unconditional counterparts. Notably the conditional models showed the best performance in nearly all settings.}
    \label{tab:t1_ade_fde}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}c|c|cc|cc|cc|cc|cc@{}}
        \toprule
        \textbf{\begin{tabular}[c]{@{}c@{}}Data\\ set\end{tabular}} &
            \textbf{Class} &
            \textbf{RED} &
            \textbf{cRED} &
            \textbf{TF} &
            \textbf{cTF} &
            \textbf{GAN} &
            \textbf{cGAN} &
            \textbf{VAE} &
            \textbf{cVAE} &
            \textbf{MoD} &
            \textbf{cMoD} \\ \midrule
        \multirow{13}{*}{\rotatebox{90}{TH\"{O}R-MAGNI Scenario~2}} &
            \begin{tabular}[c]{@{}c@{}}\emph{Carrier-}\\ \emph{Box}\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}0.64$\pm$0.07\\ 1.23$\pm$0.14\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.60$\pm$0.07\\ 1.10$\pm$0.14\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.66$\pm$0.07\\ 1.24$\pm$0.15\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.60$\pm$0.07\\ 1.10$\pm$0.13\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.76$\pm$0.07\\ 1.50$\pm$0.19\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.70$\pm$0.10\\ 1.33$\pm$0.19\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.68$\pm$0.06\\ 1.31$\pm$0.13\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.66$\pm$0.05\\ 1.26$\pm$0.11\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.81$\pm$0.11\\ 1.59$\pm$0.25\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.73$\pm$0.07\\ 1.40$\pm$0.17\end{tabular}}
            \\ \cmidrule(l){2-12} 
            &
            \begin{tabular}[c]{@{}c@{}}\emph{Carrier-}\\ \emph{Bucket}\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}0.71$\pm$0.06\\ 1.35$\pm$0.18\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.67$\pm$0.06\\ 1.21$\pm$0.15\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.65$\pm$0.05\\ 1.24$\pm$0.13\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.60$\pm$0.06\\ 1.12$\pm$0.16\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.78$\pm$0.04\\ 1.48$\pm$0.18\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.73$\pm$0.06\\ 1.37$\pm$0.14\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}\textbf{0.73}$\pm$\textbf{0.09}\\ 1.44$\pm$0.20\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}0.74$\pm$0.08\\ \textbf{1.43}$\pm$\textbf{0.19}\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}0.92$\pm$0.18\\ 1.78$\pm$0.37\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.72$\pm$0.10\\ 1.30$\pm$0.17\end{tabular}}
            \\ \cmidrule(l){2-12} 
            &
            \begin{tabular}[c]{@{}c@{}}\emph{Visitors-}\\ \emph{Alone}\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}0.81$\pm$0.05\\ 1.53$\pm$0.12\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.78$\pm$0.06\\ 1.48$\pm$0.13\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.79$\pm$0.04\\ 1.52$\pm$0.12\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.75$\pm$0.04\\ 1.45$\pm$0.14\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.88$\pm$0.07\\ 1.72$\pm$0.14\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.85$\pm$0.08\\ 1.67$\pm$0.19\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.84$\pm$0.06\\ 1.62$\pm$0.16\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.83$\pm$0.05\\ \textbf{1.61}$\pm$\textbf{0.14}\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.94$\pm$0.06\\ 1.97$\pm$0.20\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.92$\pm$0.09\\ 1.95$\pm$0.22\end{tabular}}
            \\ \cmidrule(l){2-12} 
            &
            \begin{tabular}[c]{@{}c@{}}\emph{Visitors-}\\ \emph{Group}\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.72$\pm$0.05\\ 1.34$\pm$0.17\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}\textbf{0.72}$\pm$\textbf{0.07}\\ 1.35$\pm$0.18\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}0.74$\pm$0.06\\ 1.40$\pm$0.15\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.68$\pm$0.05\\ 1.29$\pm$0.13\end{tabular}} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.80$\pm$0.08\\ 1.52$\pm$0.15\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}\textbf{0.80}$\pm$\textbf{0.06}\\ 1.57$\pm$0.16\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}0.78$\pm$0.08\\ 1.59$\pm$0.16\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.75$\pm$0.06\\ 1.56$\pm$0.13\end{tabular}} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.82$\pm$0.10\\ 1.78$\pm$0.24\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.83$\pm$0.10\\ 1.80$\pm$0.24\end{tabular}
            \\ \cmidrule(l){2-12} 
            &
            \begin{tabular}[c]{@{}c@{}}\emph{Carrier-}\\ \emph{LO}\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}0.73$\pm$0.05\\ 1.44$\pm$0.12\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.69$\pm$0.03\\ 1.38$\pm$0.10\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.69$\pm$0.05\\ 1.41$\pm$0.12\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.64$\pm$0.04\\ 1.31$\pm$0.08\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.78$\pm$0.08\\ 1.59$\pm$0.16\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.75$\pm$0.06\\ 1.56$\pm$0.13\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.77$\pm$0.07\\ 1.50$\pm$0.15\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.72$\pm$0.06\\ 1.44$\pm$0.12\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.83$\pm$0.10\\ 1.73$\pm$0.22\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.75$\pm$0.08\\ 1.61$\pm$0.19\end{tabular}}
            \\ \cmidrule(l){2-12}
            &
            \textbf{Global} &
            \begin{tabular}[c]{@{}c@{}}0.74$\pm$0.01\\ 1.41$\pm$0.04\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.71$\pm$0.03\\ 1.34$\pm$0.06\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.72$\pm$0.02\\ 1.39$\pm$0.04\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.67$\pm$0.02\\ 1.29$\pm$0.05\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.81$\pm$0.05\\ 1.59$\pm$0.09\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.78$\pm$0.05\\ 1.53$\pm$0.09\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.77$\pm$0.03\\ 1.49$\pm$0.05\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.76$\pm$0.02\\ 1.47$\pm$0.06\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}0.87$\pm$0.05 \\ 1.79$\pm$0.10\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}0.80$\pm$0.05 \\ 1.67$\pm$0.09\end{tabular}} \\ \specialrule{.2em}{.1em}{.1em}
        \multirow{9}{*}{\rotatebox{90}{SDD}} &
            \emph{Ped.} &
            \textbf{\begin{tabular}[c]{@{}c@{}}18.63$\pm$0.54\\ 37.55$\pm$1.22\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}18.76$\pm$0.54\\ 37.69$\pm$1.08\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}18.99$\pm$0.89\\ 37.60$\pm$1.76\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}19.00$\pm$0.79\\ 37.72$\pm$1.30\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}20.26$\pm$0.69\\ \textbf{40.27}$\pm$\textbf{1.25}\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}\textbf{20.21}$\pm$\textbf{0.49}\\ 40.31$\pm$0.92\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}20.92$\pm$1.25\\ 41.49$\pm$2.32\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}20.09$\pm$0.77\\ 39.90$\pm$1.44\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}19.88$\pm$0.46\\ 40.02$\pm$1.07\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}19.69$\pm$0.46\\ 39.64$\pm$1.14\end{tabular}} \\ \cmidrule(l){2-12} 
            &
            \emph{Car} &
            \begin{tabular}[c]{@{}c@{}}\textbf{8.44}$\pm$\textbf{7.48}\\ 16.63$\pm$15.03\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}8.66$\pm$7.05\\ \textbf{16.55}$\pm$\textbf{14.30}\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}9.36$\pm$6.91\\ 17.79$\pm$14.36\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}9.64$\pm$7.62\\ 18.11$\pm$15.32\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}10.99$\pm$7.39\\ 20.78$\pm$14.83\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}10.51$\pm$7.12\\ 19.55$\pm$14.23\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}10.83$\pm$7.00\\ 20.81$\pm$13.94\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}10.41$\pm$7.28\\ 18.72$\pm$13.86\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}9.95$\pm$11.05 \\ 20.61$\pm$23.07\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}8.73$\pm$9.56\\ 18.48$\pm$20.16\end{tabular}} \\ \cmidrule(l){2-12} 
            &
            \emph{Byc.} &
            \textbf{\begin{tabular}[c]{@{}c@{}}64.08$\pm$2.49\\ 137.42$\pm$5.31\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}64.38$\pm$2.53\\ 137.56$\pm$4.97\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}65.33$\pm$2.37\\ 142.08$\pm$4.60\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}64.01$\pm$2.67\\ 139.97$\pm$4.75\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}67.32$\pm$2.75\\ 145.50$\pm$5.04\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}67.04$\pm$2.41\\ 144.50$\pm$4.61\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}68.22$\pm$3.58\\ 147.00$\pm$6.32\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}67.80$\pm$3.36\\ 145.13$\pm$6.64\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}64.35$\pm$2.02\\ 142.51$\pm$4.40\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}63.60$\pm$2.02\\ 141.01$\pm$4.24\end{tabular}} \\ \cmidrule(l){2-12} 
            &
            \textbf{Global} &
            \textbf{\begin{tabular}[c]{@{}c@{}}33.95$\pm$0.91\\ 71.23$\pm$2.07\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}34.14$\pm$1.00\\ 71.38$\pm$1.99\end{tabular} &
            \begin{tabular}[c]{@{}c@{}}34.62$\pm$0.90\\ 72.87$\pm$1.70\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}34.19$\pm$1.00\\ 72.23$\pm$1.63\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}36.14$\pm$1.07\\ 75.79$\pm$1.96\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}36.01$\pm$0.75\\ 75.46$\pm$1.55\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}36.87$\pm$1.67\\ 77.09$\pm$3.08\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}36.19$\pm$1.45\\ 75.40$\pm$2.81\end{tabular}} &
            \begin{tabular}[c]{@{}c@{}}34.60$\pm$0.62 \\ 74.03$\pm$1.50\end{tabular} &
            \textbf{\begin{tabular}[c]{@{}c@{}}34.21$\pm$0.73 \\ 73.25$\pm$1.60\end{tabular}} \\ \bottomrule
        \end{tabular}%
    }
\vspace*{-2mm}
\end{table*}


% Read tables
% Magni
% Scenario 2
\pgfplotstableread[col  sep=comma]{contents/results_tab/magni/Scenario_2_top1_global_ade_latex.csv}\sctwoadetopone
\pgfplotstableread[col sep=comma]{contents/results_tab/magni/Scenario_2_top1_global_fde_latex.csv}\sctwofdetopone
\pgfplotstableread[col  sep=comma]{contents/results_tab/magni/Scenario_2_top3_global_ade_latex.csv}\sctwoadetopthree
\pgfplotstableread[col sep=comma]{contents/results_tab/magni/Scenario_2_top3_global_fde_latex.csv}\sctwofdetopthree

% Scenario 3A
\pgfplotstableread[col  sep=comma]{contents/results_tab/magni/Scenario_3A_top1_global_ade_latex.csv}\sctaadetopone
\pgfplotstableread[col sep=comma]{contents/results_tab/magni/Scenario_3A_top1_global_fde_latex.csv}\sctafdetopone
\pgfplotstableread[col  sep=comma]{contents/results_tab/magni/Scenario_3A_top3_global_ade_latex.csv}\sctaadetopthree
\pgfplotstableread[col sep=comma]{contents/results_tab/magni/Scenario_3A_top3_global_fde_latex.csv}\sctafdetopthree

% Scenario 3B
\pgfplotstableread[col  sep=comma]{contents/results_tab/magni/Scenario_3B_top1_global_ade_latex.csv}\sctbadetopone
\pgfplotstableread[col sep=comma]{contents/results_tab/magni/Scenario_3B_top1_global_fde_latex.csv}\sctbfdetopone
\pgfplotstableread[col  sep=comma]{contents/results_tab/magni/Scenario_3B_top3_global_ade_latex.csv}\sctbadetopthree
\pgfplotstableread[col sep=comma]{contents/results_tab/magni/Scenario_3B_top3_global_fde_latex.csv}\sctbfdetopthree


% sdd
\pgfplotstableread[col  sep=comma]{contents/results_tab/sdd/sdd_top1_global_ade_latex.csv}\sddadetopone
\pgfplotstableread[col sep=comma]{contents/results_tab/sdd/sdd_top1_global_fde_latex.csv}\sddfdetopone
\pgfplotstableread[col  sep=comma]{contents/results_tab/sdd/sdd_top3_global_ade_latex.csv}\sddadetopthree
\pgfplotstableread[col sep=comma]{contents/results_tab/sdd/sdd_top3_global_fde_latex.csv}\sddfdetopthree

% Scenario 2
\begin{comment}
\begin{figure}[!t]
    \centering
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train Set Ratio (\%)},
                ylabel={Top-$1$ ADE (m)},
                legend columns=2,
                grid=major,
                ymax=1.25,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[magenta, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sctwoadetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sctwoadetopone};
            \addlegendentryexpanded{RED};

            \addplot[magenta, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sctwoadetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sctwoadetopone};
            \addlegendentryexpanded{cRED};

            \addplot[black, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sctwoadetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sctwoadetopone};
            \addlegendentryexpanded{TF};

            \addplot[black, mark=asterisk]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sctwoadetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sctwoadetopone};
            \addlegendentryexpanded{cTF};

            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctwoadetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctwoadetopone};
            \addlegendentryexpanded{MoD};

            \addplot[teal, mark=|]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctwoadetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctwoadetopone};
            \addlegendentryexpanded{cMoD};
        \end{axis}
    \end{tikzpicture}
}
\hfill
\resizebox{.49\columnwidth}{!}{
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width = \columnwidth,
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$1$ FDE (m)},
            legend columns=2,
            grid=major,
            ymax=2.50,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[magenta, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sctwofdetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sctwofdetopone};
        \addlegendentryexpanded{RED};

        \addplot[magenta, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sctwofdetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sctwofdetopone};
        \addlegendentryexpanded{cRED};

        \addplot[black, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sctwofdetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sctwofdetopone};
        \addlegendentryexpanded{TF};

        \addplot[black, mark=asterisk]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sctwofdetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sctwofdetopone};
        \addlegendentryexpanded{cTF};

        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctwoadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctwofdetopone};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctwoadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctwofdetopone};
        \addlegendentryexpanded{cMoD};
        
        \end{axis}
    \end{tikzpicture}
}
\caption{Top-$1$ ADE/FDE scores of single-output deep learning models in TH\"{O}R-MAGNI Scenario 2.}
\label{fig:det_deep_learning_t1_sc2}
\end{figure}
\end{comment}

\begin{comment}
    


\begin{figure}[!t]
    \centering
    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$3$ ADE (m)},
            legend columns=2,
            grid=major,
            ymax=1.05,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[blue, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctwoadetopthree}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{VAE};

        \addplot[blue, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctwoadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{cVAE};

        \addplot[red, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctwoadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{GAN};

        \addplot[red, mark=+] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctwoadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{cGAN};

        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctwoadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctwoadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{cMoD};
        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$3$ FDE (m)},
                legend columns=2,
                grid=major,
                ymax=2.25,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[blue, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctwofdetopthree}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{VAE};

            \addplot[blue, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctwofdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{cVAE};
    
            \addplot[red, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctwofdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{GAN};
    
            \addplot[red, mark=+] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctwofdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{cGAN};

            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctwofdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{MoD};
    
            \addplot[teal, mark=|] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctwofdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{cMoD};
            
            \end{axis}
        \end{tikzpicture}
    }
    \caption{Top-$3$ ADE/FDE scores of generative deep learning models in TH\"{O}R-MAGNI Scenario 2.}
    \label{fig:gen_deep_learning_ade_sc2}
\end{figure}

\end{comment}

% \begin{figure}[!t]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             xlabel={Train set Ratio (\%)},
%             ylabel={Top-$3$ FDE (m)},
%             legend columns=2,
%             grid=major,
%             ymax=1.85,
%             xtick=data,
%         ]
        
%         \addplot[blue, mark=diamond]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctwofdetopthree}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctwofdetopthree};
%         \addlegendentryexpanded{VAE};

%         \addplot[red, mark=oplus]
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctwofdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctwofdetopthree};
%         \addlegendentryexpanded{GAN};

%         \addplot[blue, mark=triangle] 
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctwofdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctwofdetopthree};
%         \addlegendentryexpanded{cVAE};


%         \addplot[red, mark=+] 
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctwofdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctwofdetopthree};
%         \addlegendentryexpanded{cGAN};
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Top-$3$ FDE scores of generative deep learning models in TH\"{O}R-MAGNI Scenario 2.}
%     \label{fig:gen_deep_learning_fde_sc2}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[t]
\centering
%\includegraphics[clip,trim=0mm 21mm 0mm 0mm,height=26mm]{figures/quantity_res/ADE_new.pdf}
%\includegraphics[clip,trim=0mm 21mm 0mm 0mm,height=26mm]{figures/quantity_res/FDE_new.pdf}
%\includegraphics[clip,trim=0mm 0mm 0mm 0mm,height=31mm]{figures/quantity_res/Top-k ADE_new.pdf}
%\includegraphics[clip,trim=0mm 0mm 0mm 0mm,height=31mm]{figures/quantity_res/Top-k FDE_new.pdf}
\includegraphics[width=12mm, angle=90]{figures/quality_res_v2/sdd/deathCircle_0_Biker_3730535_GAN.pdf}
\includegraphics[width=12mm, angle=90]{figures/quality_res_v2/sdd/gates_1_Pedestrian_210172_GAN.pdf}
\includegraphics[height=12mm]{figures/quality_res_v2/sdd/nexus_9_Car_2360073_GAN.pdf}

\includegraphics[width=12mm, angle=90]{figures/quality_res_v2/sdd/deathCircle_0_Biker_3730535_VAE.pdf}
\includegraphics[width=12mm, angle=90]{figures/quality_res_v2/sdd/gates_1_Pedestrian_210172_VAE.pdf}
\includegraphics[height=12mm]{figures/quality_res_v2/sdd/nexus_9_Car_2360073_VAE.pdf}

\includegraphics[width=12mm, angle=90]{figures/quality_res_v2/sdd/deathCircle_0_Biker_3730535_MoD.pdf}
\includegraphics[width=12mm, angle=90]{figures/quality_res_v2/sdd/gates_1_Pedestrian_210172_MoD.pdf}
\includegraphics[height=12mm]{figures/quality_res_v2/sdd/nexus_9_Car_2360073_MoD.pdf}

\caption{Prediction examples of {\em Byciclist} (\textbf{left}), {\em Pedestrian} (\textbf{middle}) and {\em Car} (\textbf{right}) in SDD with \SI{4.8}{\second} prediction horizon.}
\label{fig:sdd_quality_res}
\vspace*{-6mm}
\end{figure*}



\begin{figure}
\centering
\includegraphics[width=.32\linewidth]{figures/compare-mods/magni/sce1_general_b1.pdf}
\includegraphics[width=.32\linewidth]{figures/compare-mods/magni/sce1_carrier_box_b1.pdf}
\includegraphics[width=.32\linewidth]{figures/compare-mods/magni/sce1_carrier_bucket_b1.pdf}
\includegraphics[width=.32\linewidth]{figures/compare-mods/magni/sce1_carrier_lo_b1.pdf}
\includegraphics[width=.32\linewidth]{figures/compare-mods/magni/sce1_visitors_alone_b1.pdf}
\includegraphics[width=.32\linewidth]{figures/compare-mods/magni/sce1_visitors_g_b1.pdf}

\caption{General and class-conditioned CLiFF-maps in Scenario~2 of the TH\"{O}R-MAGNI dataset, shown in colored arrows. \textbf{Top row from left to right:} combination of all classes, {\em Carrier--Box}, {\em Carrier--Bucket}. \textbf{Bottom row from left to right:} {\em Carrier--Large Object}, {\em Visitors--Alone}, and {\em Visitors--Group}. The motion patterns represented in CLiFF-maps exhibit distinct characteristics across different classes.}
\label{fig:CLiFF-mapMAGNI}
\vspace*{-7mm}
\end{figure}



% Scenario 3A



% \begin{figure}[!t]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             xlabel={Train set Ratio (\%)},
%             ylabel={Top-$1$ FDE (m)},
%             legend columns=2,
%             grid=major,
%             ymax=2.05,
%             xtick=data,
%         ]
        
%         \addplot[magenta, mark=diamond]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sctafdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sctafdetopone};
%         \addlegendentryexpanded{RED};

%         \addplot[black, mark=oplus]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sctafdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sctafdetopone};
%         \addlegendentryexpanded{TF};

%         %\addplot[blue, mark=square]
%         %plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctafdetopone}; 
%         %table[x expr={100 - \thisrow{test_ratio}}, y=CliFF-LHMP_avg]{\sctafdetopone};
%         %\addlegendentryexpanded{CliFF-LHMP};


%         \addplot[magenta, mark=triangle] 
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sctafdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sctafdetopone};
%         \addlegendentryexpanded{cRED};


%         \addplot[black, mark=asterisk]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sctafdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sctafdetopone};
%         \addlegendentryexpanded{cTF};

%         %\addplot[blue, mark=|]
%         %plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctafdetopone}; 
%         %table[x expr={100 - \thisrow{test_ratio}}, y=cCliFF-LHMP_avg]{\sctafdetopone};
%         %\addlegendentryexpanded{cCliFF-LHMP};
        
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Top-$1$ FDE scores of single-output deep learning models in TH\"{O}R-MAGNI Scenario 3A.}
%     \label{fig:det_deep_learning_fde_sc3a}
% \end{figure}






% \begin{figure}[!t]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             xlabel={Train set Ratio (\%)},
%             ylabel={Top-$3$ FDE (m)},
%             legend columns=2,
%             grid=major,
%             ymax=1.70,
%             xtick=data,
%         ]
        
%         \addplot[blue, mark=diamond]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctafdetopthree}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctafdetopthree};
%         \addlegendentryexpanded{VAE};

%         \addplot[red, mark=oplus]
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctafdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctafdetopthree};
%         \addlegendentryexpanded{GAN};

%         \addplot[blue, mark=triangle] 
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctafdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctafdetopthree};
%         \addlegendentryexpanded{cVAE};


%         \addplot[red, mark=+] 
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctafdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctafdetopthree};
%         \addlegendentryexpanded{cGAN};
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Top-$3$ FDE scores of generative deep learning models in TH\"{O}R-MAGNI Scenario 3A.}
%     \label{fig:gen_deep_learning_fde_sc3a}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
    

% Scenario 3B
\begin{figure}[!t]
    \centering
    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$1$ ADE (m)},
            legend columns=2,
            grid=major,
            ymax=1.15,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[magenta, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sctbadetopone};
        \addlegendentryexpanded{RED};

        \addplot[magenta, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sctbadetopone};
        \addlegendentryexpanded{cRED};

        \addplot[black, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sctbadetopone};
        \addlegendentryexpanded{TF};

        \addplot[black, mark=asterisk]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sctbadetopone};
        \addlegendentryexpanded{cTF};

        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctbadetopone};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctbadetopone};
        \addlegendentryexpanded{cMoD};
        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$1$ FDE (m)},
                legend columns=2,
                grid=major,
                ymax=2.5,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[magenta, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sctbfdetopone};
            \addlegendentryexpanded{RED};

            \addplot[magenta, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sctbfdetopone};
            \addlegendentryexpanded{cRED};
    
            \addplot[black, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sctbfdetopone};
            \addlegendentryexpanded{TF};

            \addplot[black, mark=asterisk]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sctbfdetopone};
            \addlegendentryexpanded{cTF};
    
            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctbfdetopone};
            \addlegendentryexpanded{MoD};
    
            \addplot[teal, mark=|]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctbfdetopone};
            \addlegendentryexpanded{cMoD};
            
            \end{axis}
        \end{tikzpicture}
    }
    \caption{Top-$1$ ADE/FDE scores of single-output deep learning models in TH\"{O}R-MAGNI Scenario 3B.}
    \label{fig:det_deep_learning_ade_sc3b}
\end{figure}

\end{comment}


% \begin{figure}[!t]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             xlabel={Train set Ratio (\%)},
%             ylabel={Top-$1$ FDE (m)},
%             legend columns=2,
%             grid=major,
%             ymax=2.1,
%             xtick=data,
%         ]
        
%         \addplot[magenta, mark=diamond]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sctbfdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sctbfdetopone};
%         \addlegendentryexpanded{RED};

%         \addplot[black, mark=oplus]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sctbfdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sctbfdetopone};
%         \addlegendentryexpanded{TF};

%         %\addplot[blue, mark=square]
%         %plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctbfdetopone}; 
%         %table[x expr={100 - \thisrow{test_ratio}}, y=CliFF-LHMP_avg]{\sctbfdetopone};
%         %\addlegendentryexpanded{CliFF-LHMP};


%         \addplot[magenta, mark=triangle] 
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sctbfdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sctbfdetopone};
%         \addlegendentryexpanded{cRED};


%         \addplot[black, mark=asterisk]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sctbfdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sctbfdetopone};
%         \addlegendentryexpanded{cTF};

%         %\addplot[blue, mark=|]
%         %plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctbfdetopone}; 
%         %table[x expr={100 - \thisrow{test_ratio}}, y=cCliFF-LHMP_avg]{\sctbfdetopone};
%         %\addlegendentryexpanded{cCliFF-LHMP};
        
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Top-$1$ FDE scores of single-output deep learning models in TH\"{O}R-MAGNI Scenario 3B.}
%     \label{fig:det_deep_learning_fde_sc3b}
% \end{figure}

\begin{comment}

\begin{figure}[!t]
    \centering
    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$3$ ADE (m)},
            legend columns=2,
            grid=major,
            ymax=1.0,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[blue, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctbadetopthree}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctbadetopthree};
        \addlegendentryexpanded{VAE};

        \addplot[blue, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctbadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctbadetopthree};
        \addlegendentryexpanded{cVAE};

        \addplot[red, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctbadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctbadetopthree};
        \addlegendentryexpanded{GAN};

        \addplot[red, mark=+] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctbadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctbadetopthree};
        \addlegendentryexpanded{cGAN};

        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctafdetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctbadetopthree};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctafdetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctbadetopthree};
        \addlegendentryexpanded{cMoD};

        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$3$ FDE (m)},
                legend columns=2,
                grid=major,
                ymax=2.00,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[blue, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctbfdetopthree}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctbfdetopthree};
            \addlegendentryexpanded{VAE};

            \addplot[blue, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctbfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctbfdetopthree};
            \addlegendentryexpanded{cVAE};
    
            \addplot[red, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctbfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctbfdetopthree};
            \addlegendentryexpanded{GAN};
    
            \addplot[red, mark=+] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctbfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctbfdetopthree};
            \addlegendentryexpanded{cGAN};

            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctafdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctafdetopthree};
            \addlegendentryexpanded{MoD};
    
            \addplot[teal, mark=|] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctafdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctafdetopthree};
            \addlegendentryexpanded{cMoD};

            
            \end{axis}
        \end{tikzpicture}

    }
    \caption{Top-$3$ ADE/FDE scores of generative deep learning models in TH\"{O}R-MAGNI Scenario 3B.}
    \label{fig:gen_deep_learning_ade_sc3b}
\end{figure}

\end{comment}

% \begin{figure}[!t]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             xlabel={Train set Ratio (\%)},
%             ylabel={Top-$3$ FDE (m)},
%             legend columns=2,
%             grid=major,
%             ymax=1.80,
%             xtick=data,
%         ]
        
%         \addplot[blue, mark=diamond]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctbfdetopthree}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctbfdetopthree};
%         \addlegendentryexpanded{VAE};

%         \addplot[red, mark=oplus]
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctbfdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctbfdetopthree};
%         \addlegendentryexpanded{GAN};

%         \addplot[blue, mark=triangle] 
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctbfdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctbfdetopthree};
%         \addlegendentryexpanded{cVAE};


%         \addplot[red, mark=+] 
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctbfdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctbfdetopthree};
%         \addlegendentryexpanded{cGAN};
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Top-$3$ FDE scores of generative deep learning models in TH\"{O}R-MAGNI Scenario 3B.}
%     \label{fig:gen_deep_learning_fde_sc3b}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\begin{figure}[!t]
    \centering
    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train Set Ratio (\%)},
            ylabel={Top-$1$ ADE (m)},
            legend columns=2,
            grid=major,
            ymax=39,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[magenta, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sddadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sddadetopone};
        \addlegendentryexpanded{RED};

        \addplot[magenta, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sddadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sddadetopone};
        \addlegendentryexpanded{cRED};

        \addplot[black, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sddadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sddadetopone};
        \addlegendentryexpanded{TF};

        \addplot[black, mark=asterisk]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sddadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sddadetopone};
        \addlegendentryexpanded{cTF};

        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctwoadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sddadetopone};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sddadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sddadetopone};
        \addlegendentryexpanded{cMoD};
        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$1$ FDE (m)},
                legend columns=2,
                grid=major,
                ymax=80,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[magenta, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sddfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sddfdetopone};
            \addlegendentryexpanded{RED};

            \addplot[magenta, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sddfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sddfdetopone};
            \addlegendentryexpanded{cRED};

    
            \addplot[black, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sddfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sddfdetopone};
            \addlegendentryexpanded{TF};


            \addplot[black, mark=asterisk]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sddfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sddfdetopone};
            \addlegendentryexpanded{cTF};

    
            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctwoadetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sddfdetopone};
            \addlegendentryexpanded{MoD};

    
            \addplot[teal, mark=|]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctwoadetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sddfdetopone};
            \addlegendentryexpanded{cMoD};
            
            \end{axis}
        \end{tikzpicture}
    }
    \caption{Top-$1$ ADE/FDE scores of single-output deep learning models in SDD.}
    \label{fig:det_deep_learning_ade_sdd}
\end{figure}
\end{comment}


% \begin{figure}[!t]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             xlabel={Train set Ratio (\%)},
%             ylabel={Top-$1$ FDE (m)},
%             legend columns=2,
%             grid=major,
%             ymax=79,
%             xtick=data,
%         ]
        
%         \addplot[magenta, mark=diamond]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sddfdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sddfdetopone};
%         \addlegendentryexpanded{RED};

%         \addplot[black, mark=oplus]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sddfdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sddfdetopone};
%         \addlegendentryexpanded{TF};

%         % \addplot[blue, mark=square]
%         % plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctwoadetopone}; 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=CliFF-LHMP_avg]{\sddfdetopone};
%         % \addlegendentryexpanded{CliFF-LHMP};


%         \addplot[magenta, mark=triangle] 
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sddfdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sddfdetopone};
%         \addlegendentryexpanded{cRED};


%         \addplot[black, mark=asterisk]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sddfdetopone}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sddfdetopone};
%         \addlegendentryexpanded{cTF};

%         % \addplot[blue, mark=|]
%         % plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctwoadetopone}; 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cCliFF-LHMP_avg]{\sddfdetopone};
%         % \addlegendentryexpanded{cCliFF-LHMP};
        
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Top-$1$ FDE scores of single-output deep learning models in SDD.}
%     \label{fig:det_deep_learning_fde_sdd}
% \end{figure}

\begin{comment}
    


\begin{figure}[!t]
    \centering
    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$3$ ADE (m)},
            legend columns=2,
            grid=major,
            ymax=36,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[blue, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sddadetopthree}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sddadetopthree};
        \addlegendentryexpanded{VAE};

        \addplot[blue, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sddadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sddadetopthree};
        \addlegendentryexpanded{cVAE};

        \addplot[red, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sddadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sddadetopthree};
        \addlegendentryexpanded{GAN};

        \addplot[red, mark=+] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sddadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sddadetopthree};
        \addlegendentryexpanded{cGAN};


        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sddadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sddadetopthree};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sddadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sddadetopthree};
        \addlegendentryexpanded{cMoD};

        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$3$ FDE (m)},
                legend columns=2,
                grid=major,
                ymax=75,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[blue, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sddfdetopthree}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sddfdetopthree};
            \addlegendentryexpanded{VAE};

            \addplot[blue, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sddfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sddfdetopthree};
            \addlegendentryexpanded{cVAE};

            \addplot[red, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sddfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sddfdetopthree};
            \addlegendentryexpanded{GAN};
    
            \addplot[red, mark=+] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sddfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sddfdetopthree};
            \addlegendentryexpanded{cGAN};

            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sddfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sddfdetopthree};
            \addlegendentryexpanded{MoD};
    
            \addplot[teal, mark=|] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sddfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sddfdetopthree};
            \addlegendentryexpanded{cMoD};


            
            \end{axis}
        \end{tikzpicture}
    }
    \caption{Top-$3$ ADE/FDE scores of generative deep learning models in SDD.}
    \label{fig:gen_deep_learning_ade_sdd}
\end{figure}

\end{comment}

% \begin{figure}[!t]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             xlabel={Train set Ratio (\%)},
%             ylabel={Top-$3$ FDE (m)},
%             legend columns=2,
%             grid=major,
%             ymax=72,
%             xtick=data,
%         ]
        
%         \addplot[blue, mark=diamond]
%         plot [error bars/.cd, y dir=both, y explicit]
%         % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sddfdetopthree}; 
%         table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sddfdetopthree};
%         \addlegendentryexpanded{VAE};

%         \addplot[red, mark=oplus]
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sddfdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sddfdetopthree};
%         \addlegendentryexpanded{GAN};

%         \addplot[blue, mark=triangle] 
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sddfdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sddfdetopthree};
%         \addlegendentryexpanded{cVAE};


%         \addplot[red, mark=+] 
%         plot [error bars/.cd, y dir=both, y explicit] 
%         % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sddfdetopthree};
%         table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sddfdetopthree};
%         \addlegendentryexpanded{cGAN};
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Top-$3$ FDE scores of generative deep learning models in SDD.}
%     \label{fig:gen_deep_learning_fde_sdd}
% \end{figure}

%TODO: fix this section
%In this section, we present the results obtained in the TH\"{O}R-MAGNI and SDD datasets with both deep learning-based methods and an MoD-based method. The performance is evaluated with both quantitative and qualitative analysis. 

%\cref{tab:t1_ade_fde} shows the experimental results of each class on Scenario 2 of TH\"{O}R-MAGNI and SDD datasets. On TH\"{O}R-MAGNI dataset, both deep learning based methods and the MoD-based method in general achieves better results with the class conditioned version. When predicting trajectories in the class of \emph{Visitors-Group}, because as shown in \cref{fig:CLiFF-mapMAGNI}, the motion patterns of \emph{Visitors-Group} (\textbf{bottom right}) is not clear, both deep learning methods and MoD-based method fail to improve accuracy with the class attribute.

%For SDD dataset, where class is imbalance, single-output based methods (TF and RED) do not benefit from the class attribute. 


%The Top-$1$ results of single-output methods for TH\"{O}R-MAGNI scenario 3A and 3B are shown in \cref{fig:det_deep_learning_sc3ab}.



% Tiago
We analyzed a series of experiments on the TH\"{O}R-MAGNI and SDD datasets. The main goals of these analyses are (1) to demonstrate the difference in trajectory prediction performance when using class attributes, and (2) to evaluate trajectory prediction performance based on the specific characteristics of the dataset. The latter provides insight into which trajectory prediction method is the most 
appropriate for a particular application.
Due to space limitations, we only report the results for TH\"{O}R-MAGNI Scenario~2 in \cref{tab:t1_ade_fde}, \cref{fig:CLiFF-mapMAGNI} and \cref{fig:magni_quality_res}, and for Scenarios 3A and 3B in \cref{fig:det_deep_learning_sc3ab}. We observe similar trends in all scenarios.

\subsection{Accuracy Analysis Conditioned on Class Balance}\label{sec:acc}
\cref{tab:t1_ade_fde} shows the prediction accuracy results separately for each class on Scenario~2 of the TH\"{O}R-MAGNI and SDD datasets. It also shows the global results for all trajectories (last rows for each dataset).
A broad view of the TH\"{O}R-MAGNI results shows that conditional methods outperform their unconditional counterparts regardless of the
type of method (deep learning and MoD). When predicting trajectories from the {\em Visitors--Group}, this difference 
is least pronounced. We speculate that this may be due to the fact that the motion patterns of these agents 
are less structured compared to the other classes, as shown in~\cref{fig:CLiFF-mapMAGNI}. This also highlights the importance of suitable class labels, such that each class encompasses specific motion patterns, and dataset-imposed classes may not always do so.
For the imbalanced dataset (SDD), deep learning 
methods face the challenge of identifying a representative number of different motion patterns within each class. This difficulty is most pronounced in single-output deep learning methods (RED and TF). In contrast, cMoD is less sensitive to class proportions and is able to use 
class information for more accurate predictions. 
In summary, we highlight two key points: (1) the superiority of deep learning methods over MoD-based approaches in balanced 
datasets like TH\"{O}R-MAGNI, and (2) the appropriateness of conditional MoD over deep generative methods (cGAN, cVAE) 
for imbalanced datasets like SDD.


%%%% This part is writing why class-conditioned MoD can works better than general ones.
In the MoD-aware predictor, class-conditioned CLiFF-LHMP outperforms general CLiFF-LHMP in both TH\"{O}R-MAGNI and SDD datasets. In TH\"{O}R-MAGNI, the main differences between classes are observed in the spatial patterns, as shown in \cref{fig:CLiFF-mapMAGNI}. As expected, the improvement in prediction accuracy was more pronounced in cases where the motion pattern of a specific role was more distinctly different from the general motion pattern. In SDD, variances in speed are observed among different classes, as depicted in \cref{fig:CLiFF-mapSDD}. \cref{fig:point-example-sdd} exemplifies how class-conditioned CLiFF-maps differ from the general ones. A single CLiFF-map cannot accurately model the differences among multiple classes, which causes inaccurate predictions compared with the class-conditioned MoD-aware method.


% THOR-MAGNI balanced: 
% 1) cMoD outperforms in Top-$1$ ADE for low data regimes (10%) connection with cold start
% 2) Deep generative models are globally better for sampling multiple  plausible future trajectories (Top-$3$ metrics)
% MoD better for imbalanced datasets when compared to deep generative models.
\subsection{Data Efficiency Analysis}\label{sec:data_eff}
To study the impact of the amount of data available during training on the performance of each model, we perform a data efficiency analysis. The goal is to identify the optimal models for different data settings. \cref{fig:det_deep_learning_sc3ab} shows the performance of single-output methods (RED, TF, and CLiFF-LHMP and their respective conditioned variants) in TH\"{O}R-MAGNI Scenarios 3A and 3B. As expected, the performance of the deep learning methods degrades with reduced training data, while the MoD approaches (MoD and cMoD) are more stable across different data regimes.
Moreover, class-conditioned CLiFF-LHMP (cMoD) outperforms deep learning baselines in Top-$1$ ADE for low data regimes (10\% of data available during training). These results reveal the preference for MoD-based methods in scenarios with limited training data. \cref{fig:gen_deep_learning_ade_sc23absdd} presents the performance of multiple-output methods (VAE, GAN, and CLiFF-LHMP, along with their respective conditioned variants) on the TH\"{O}R-MAGNI and SDD datasets. In TH\"{O}R-MAGNI, deep generative methods prove more effective in generating one out of $K$ trajectories compared to MoD-based methods. Conversely, in the imbalanced dataset SDD, MoD-based methods consistently outperform deep generative methods across all train set ratios. This underscores the preference for MoD-based trajectory predictors in imbalanced datasets.

\begin{figure}[!t]
    \centering
    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$1$ ADE (m)},
            label style={font=\Large},
            tick label style={font=\Large},
            legend columns=2,
            grid=major,
            ymax=1.2,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[magenta, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sctaadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sctaadetopone};
        \addlegendentryexpanded{RED};

        \addplot[magenta, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sctaadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sctaadetopone};
        \addlegendentryexpanded{cRED};

        \addplot[black, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sctaadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sctaadetopone};
        \addlegendentryexpanded{TF};


        \addplot[black, mark=asterisk]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sctaadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sctaadetopone};
        \addlegendentryexpanded{cTF};

        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctaadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctaadetopone};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctaadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctaadetopone};
        \addlegendentryexpanded{cMoD};
        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$1$ FDE (m)},
                label style={font=\Large},
                tick label style={font=\Large},
                legend columns=2,
                grid=major,
                ymax=2.50,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[magenta, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sctafdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sctafdetopone};
            \addlegendentryexpanded{RED};

            \addplot[magenta, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sctafdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sctafdetopone};
            \addlegendentryexpanded{cRED};
    
            \addplot[black, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sctafdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sctafdetopone};
            \addlegendentryexpanded{TF};

            \addplot[black, mark=asterisk]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sctafdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sctafdetopone};
            \addlegendentryexpanded{cTF};
    
            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctafdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctafdetopone};
            \addlegendentryexpanded{MoD};
    
            \addplot[teal, mark=|]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctafdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctafdetopone};
            \addlegendentryexpanded{cMoD};
            
            \end{axis}
        \end{tikzpicture}
    }

    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$1$ ADE (m)},
            label style={font=\Large},
            tick label style={font=\Large},
            legend columns=2,
            grid=major,
            ymax=1.15,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[magenta, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sctbadetopone};
        \addlegendentryexpanded{RED};

        \addplot[magenta, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sctbadetopone};
        \addlegendentryexpanded{cRED};

        \addplot[black, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sctbadetopone};
        \addlegendentryexpanded{TF};

        \addplot[black, mark=asterisk]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sctbadetopone};
        \addlegendentryexpanded{cTF};

        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctbadetopone};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctbadetopone}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctbadetopone};
        \addlegendentryexpanded{cMoD};
        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$1$ FDE (m)},
                label style={font=\Large},
                tick label style={font=\Large},
                legend columns=2,
                grid=major,
                ymax=2.5,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}},
            ]
            
            \addplot[magenta, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg, y error plus=LSTM_std, y error minus=LSTM_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=LSTM_avg]{\sctbfdetopone};
            \addlegendentryexpanded{RED};

            \addplot[magenta, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg, y error plus=cLSTM_std, y error minus=cLSTM_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cLSTM_avg]{\sctbfdetopone};
            \addlegendentryexpanded{cRED};
    
            \addplot[black, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg, y error plus=TF_std, y error minus=TF_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=TF_avg]{\sctbfdetopone};
            \addlegendentryexpanded{TF};

            \addplot[black, mark=asterisk]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg, y error plus=cTF_std, y error minus=cTF_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cTF_avg]{\sctbfdetopone};
            \addlegendentryexpanded{cTF};
    
            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=CliFFf-LHMP_avg, y error plus=CliFFf-LHMP_std, y error minus=CliFFf-LHMP_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctbfdetopone};
            \addlegendentryexpanded{MoD};
    
            \addplot[teal, mark=|]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=cLHMP_avg, y error plus=cLHMP_std, y error minus=cLHMP_std]{\sctbfdetopone}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctbfdetopone};
            \addlegendentryexpanded{cMoD};
            
            \end{axis}
        \end{tikzpicture}
    }
    
    \caption{Top-$1$ ADE/FDE scores in TH\"{O}R-MAGNI Scenario~3A (\textbf{top row}) and 3B (\textbf{bottom row}). As TH\"{O}R-MAGNI is class-balanced, deep learning methods outperform the MoD approaches. With reduced training data, the performance of deep learning methods degrades, whereas MoD approaches (MoD and cMoD) remain stable across varying data regimes.}
    \label{fig:det_deep_learning_sc3ab}
    \vspace*{-6mm}
\end{figure}

\begin{figure}[t]
    \centering
    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$3$ ADE (m)},
            label style={font=\Large},
            tick label style={font=\Large},
            legend columns=2,
            grid=major,
            ymax=1.05,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[blue, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctwoadetopthree}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{VAE};

        \addplot[blue, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctwoadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{cVAE};

        \addplot[red, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctwoadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{GAN};

        \addplot[red, mark=+] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctwoadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{cGAN};

        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctwoadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctwoadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctwoadetopthree};
        \addlegendentryexpanded{cMoD};
        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$3$ FDE (m)},
                label style={font=\Large},
                tick label style={font=\Large},
                legend columns=2,
                grid=major,
                ymax=2.25,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[blue, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctwofdetopthree}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{VAE};

            \addplot[blue, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctwofdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{cVAE};
    
            \addplot[red, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctwofdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{GAN};
    
            \addplot[red, mark=+] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctwofdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{cGAN};

            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctwofdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{MoD};
    
            \addplot[teal, mark=|] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctwofdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctwofdetopthree};
            \addlegendentryexpanded{cMoD};
            
            \end{axis}
        \end{tikzpicture}
    }

    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$3$ ADE (m)},
            label style={font=\Large},
            tick label style={font=\Large},
            legend columns=2,
            grid=major,
            ymax=0.95,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[blue, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctaadetopthree}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctaadetopthree};
        \addlegendentryexpanded{VAE};

        \addplot[blue, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctaadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctaadetopthree};
        \addlegendentryexpanded{cVAE};

        \addplot[red, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctaadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctaadetopthree};
        \addlegendentryexpanded{GAN};

        \addplot[red, mark=+] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctaadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctaadetopthree};
        \addlegendentryexpanded{cGAN};

        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctafdetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctaadetopthree};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctafdetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctaadetopthree};
        \addlegendentryexpanded{cMoD};
        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$3$ FDE (m)},
                label style={font=\Large},
                tick label style={font=\Large},
                legend columns=2,
                grid=major,
                ymax=2.00,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[blue, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctafdetopthree}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctafdetopthree};
            \addlegendentryexpanded{VAE};

            \addplot[blue, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctafdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctafdetopthree};
            \addlegendentryexpanded{cVAE};
    
            \addplot[red, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctafdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctafdetopthree};
            \addlegendentryexpanded{GAN};
    
            \addplot[red, mark=+] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctafdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctafdetopthree};
            \addlegendentryexpanded{cGAN};

            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctafdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctafdetopthree};
            \addlegendentryexpanded{MoD};
    
            \addplot[teal, mark=|] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctafdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctafdetopthree};
            \addlegendentryexpanded{cMoD};
            
            \end{axis}
        \end{tikzpicture}
    }

    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$3$ ADE (m)},
            label style={font=\Large},
            tick label style={font=\Large},
            legend columns=2,
            grid=major,
            ymax=1.0,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[blue, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctbadetopthree}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctbadetopthree};
        \addlegendentryexpanded{VAE};

        \addplot[blue, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctbadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctbadetopthree};
        \addlegendentryexpanded{cVAE};

        \addplot[red, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctbadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctbadetopthree};
        \addlegendentryexpanded{GAN};

        \addplot[red, mark=+] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctbadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctbadetopthree};
        \addlegendentryexpanded{cGAN};

        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctafdetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctbadetopthree};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctafdetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctbadetopthree};
        \addlegendentryexpanded{cMoD};

        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$3$ FDE (m)},
                label style={font=\Large},
                tick label style={font=\Large},
                legend columns=2,
                grid=major,
                ymax=2.00,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[blue, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sctbfdetopthree}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sctbfdetopthree};
            \addlegendentryexpanded{VAE};

            \addplot[blue, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sctbfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sctbfdetopthree};
            \addlegendentryexpanded{cVAE};
    
            \addplot[red, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctbfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sctbfdetopthree};
            \addlegendentryexpanded{GAN};
    
            \addplot[red, mark=+] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctbfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sctbfdetopthree};
            \addlegendentryexpanded{cGAN};

            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sctafdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sctafdetopthree};
            \addlegendentryexpanded{MoD};
    
            \addplot[teal, mark=|] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sctafdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sctafdetopthree};
            \addlegendentryexpanded{cMoD};

            
            \end{axis}
        \end{tikzpicture}

    }

    \resizebox{.49\columnwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xlabel={Train set Ratio (\%)},
            ylabel={Top-$3$ ADE (m)},
            label style={font=\Large},
            tick label style={font=\Large},
            legend columns=2,
            grid=major,
            ymax=36,
            xtick=data,
            legend style={nodes={scale=1.9, transform shape}}, 
        ]
        
        \addplot[blue, mark=diamond]
        plot [error bars/.cd, y dir=both, y explicit]
        % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sddadetopthree}; 
        table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sddadetopthree};
        \addlegendentryexpanded{VAE};

        \addplot[blue, mark=triangle] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sddadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sddadetopthree};
        \addlegendentryexpanded{cVAE};

        \addplot[red, mark=oplus]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sddadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sddadetopthree};
        \addlegendentryexpanded{GAN};

        \addplot[red, mark=+] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sddadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sddadetopthree};
        \addlegendentryexpanded{cGAN};


        \addplot[teal, mark=square]
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sddadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sddadetopthree};
        \addlegendentryexpanded{MoD};

        \addplot[teal, mark=|] 
        plot [error bars/.cd, y dir=both, y explicit] 
        % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sddadetopthree};
        table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sddadetopthree};
        \addlegendentryexpanded{cMoD};

        
        \end{axis}
    \end{tikzpicture}
    }
    \resizebox{.49\columnwidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Train set Ratio (\%)},
                ylabel={Top-$3$ FDE (m)},
                label style={font=\Large},
                tick label style={font=\Large},
                legend columns=2,
                grid=major,
                ymax=75,
                xtick=data,
                legend style={nodes={scale=1.9, transform shape}}, 
            ]
            
            \addplot[blue, mark=diamond]
            plot [error bars/.cd, y dir=both, y explicit]
            % table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg, y error plus=VAE_std, y error minus=VAE_std]{\sddfdetopthree}; 
            table[x expr={100 - \thisrow{test_ratio}}, y=VAE_avg]{\sddfdetopthree};
            \addlegendentryexpanded{VAE};

            \addplot[blue, mark=triangle] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg, y error plus=cVAE_std, y error minus=cVAE_std] {\sddfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cVAE_avg]{\sddfdetopthree};
            \addlegendentryexpanded{cVAE};

            \addplot[red, mark=oplus]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sddfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg]{\sddfdetopthree};
            \addlegendentryexpanded{GAN};
    
            \addplot[red, mark=+] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sddfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg]{\sddfdetopthree};
            \addlegendentryexpanded{cGAN};

            \addplot[teal, mark=square]
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=GAN_avg, y error plus=GAN_std, y error minus=GAN_std] {\sddfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=MoD_avg]{\sddfdetopthree};
            \addlegendentryexpanded{MoD};
    
            \addplot[teal, mark=|] 
            plot [error bars/.cd, y dir=both, y explicit] 
            % table[x expr={100 - \thisrow{test_ratio}}, y=cGAN_avg, y error plus=cGAN_std, y error minus=cGAN_std] {\sddfdetopthree};
            table[x expr={100 - \thisrow{test_ratio}}, y=cMoD_avg]{\sddfdetopthree};
            \addlegendentryexpanded{cMoD};
            
            \end{axis}
        \end{tikzpicture}
    }

    \caption{Top-$3$ ADE/FDE scores in TH\"{O}R-MAGNI Scenario~2 (\textbf{top row}), 3A (\textbf{second row}), 3B (\textbf{third row}) and SDD (\textbf{bottom row}). Deep generative methods outperform MoD approaches in the class-balanced dataset TH\"{O}R-MAGNI. In the imbalanced dataset SDD, MoD approaches consistently outperform deep generative methods across varying data regimes.}
    \label{fig:gen_deep_learning_ade_sc23absdd}
    \vspace*{-1mm}
\end{figure}

\subsection{Qualitative Results}

% Qualitative results
We provide qualitative Top-$1$ trajectory prediction comparisons for each multiple-output approach in \cref{fig:sdd_quality_res} and for each single-output method in \cref{fig:magni_quality_res} for the SDD and TH\"{O}R-MAGNI datasets, respectively. For both datasets, conditioned methods are more accurate than their unconditional counterparts. On the SDD dataset, which is characterized by imbalanced classes, cMoD is the most effective compared to deep learning methods. On the TH\"{O}R-MAGNI dataset, we observed that conditioned deep learning methods outperform both unconditional deep learning methods and the MoD approaches, which is consistent with the quantitative results.

\begin{figure}[!t]
\centering
%\includegraphics[clip,trim=0mm 21mm 0mm 0mm,height=26mm]{figures/quantity_res/ADE_new.pdf}
%\includegraphics[clip,trim=0mm 21mm 0mm 0mm,height=26mm]{figures/quantity_res/FDE_new.pdf}
%\includegraphics[clip,trim=0mm 0mm 0mm 0mm,height=31mm]{figures/quantity_res/Top-k ADE_new.pdf}
%\includegraphics[clip,trim=0mm 0mm 0mm 0mm,height=31mm]{figures/quantity_res/Top-k FDE_new.pdf}
\includegraphics[width=.48\linewidth]{figures/quality_res_v2/magni/sce1_carrier_box_11068.pdf}
\includegraphics[width=.48\linewidth]{figures/quality_res_v2/magni/sce1_carrier_bucket_12131.pdf}
\includegraphics[width=.48\linewidth]{figures/quality_res_v2/magni/sce1_visitors_alone_14345.pdf}
\includegraphics[width=.48\linewidth]{figures/quality_res_v2/magni/sce1_carrier_lo_13358.pdf}
\caption{Prediction examples of {\em Carrier--Box} (\textbf{top left}), {\em Carrier--Bucket} (\textbf{top right}), {\em Visitors--Alone} (\textbf{bottom left}) and {\em Carrier--Large Object} (\textbf{bottom right}) in TH\"{O}R-MAGNI with \SI{4.8}{\second} prediction horizon.}
\label{fig:magni_quality_res}
\vspace*{-4mm}
\end{figure}

==> contents/6_conclusion.tex <==
\section{CONCLUSION} \label{section-conclusion}
%In this study, we demonstrate the role of class attributes in enhancing the prediction accuracy of several trajectory prediction methods. Through a comprehensive comparative analysis, encompassing deep learning approaches and MoD-aware methods, our findings consistently highlight the superior performance of class-conditioned methods over their unconditioned counterparts. We conducted these experiments on two distinct datasets, where we found that deep learning methods face challenges in effectively leveraging the potential of the class attribute in imbalanced datasets such as SDD. In contrast, MoD-aware methods demonstrate the ability to benefit from the class attribute, irrespective of the dataset's nature. In balanced datasets like TH\"{O}R-MAGNI, deep learning methods show superiority over the MoD-based approach. Additionally, in applications with limited data during training, i.e., low data regimes (e.g. cold start of a robot in a new unseen environment), MoD-based methods are preferable over deep learning methods.

The challenge of making accurate trajectory predictions in dynamic environments is further complicated when facing heterogeneous agents with diverse dynamics and distinct motion patterns. Considering the classes of agents can help lowering the uncertainty in motion forecasts, an issue that arises when attempting to generalize across different classes. In this paper, we analyze how prior art in deep learning-based and pattern-based prediction can be adapted to consider class labels. We conclude that class-conditioned methods generally outperform their unconditioned counterparts. The choice of a specific method, on the other hand, strongly depends on the available training data: in new environments with limited data, as well as in such environments where some classes are underrepresented (sometimes critically so, e.g., vulnerable road users in automated driving), pattern-based methods may have an edge over the deep learning models. In future work, we intend to extend this analysis to upstream class detection, and look into unsupervised class definition using trajectory and dynamics clustering.

==> revision-contents/commands.tex <==
%
% Common abbreviations
%
\newcommand{\ie}{i.\,e.}
\newcommand{\eg}{e.\,g.}
\newcommand{\etc}{etc.}



%
% Environments
%
\newtheorem{definition}{Definition}

%
% Editing commands
%
\newcommand{\citn}{{\color{red}[Citation needed]}} % citation to be addedd
\newcommand{\refn}{{\color{red}[Reference needed]}} % reference to a forward section
\newcommand{\reflect}[2][]{{\color{blue}[\ifthenelse{\equal{#1}{}}{}{(#1) }#2]}} % part requires reflection - optional argument to specify who added the comment
\newcommand{\tbd}{{\color{orange}TBD}} % to be done
\newcommand{\com}[2][]{{\color{green}[\ifthenelse{\equal{#1}{}}{}{(#1) }#2]}} % comment - optional argument to specify who added the comment
\newcommand{\todo}[1]{{\color{red}TODO:#1}}
\newcommand{\wip}{{\color{orange}WIP}}
\newcommand{\rev}{{\color{yellow}Revision}}
\newcommand{\done}{{\color{green}Done}}
\newcommand{\att}[2]{{\color{orange}{\textbf{[(@#1) #2}]}}} %"att" for targeted todos
